State of the Art of the Intra-Task Dynamic Voltage and Frequency Scaling Technique

In recent years there has been an increasing use of embedded systems because of advances in technology, the reduction of the costs of electronic equipment and mainly the popularity of mobile devices. Many of these systems implement low power consumption policies to extend their autonomy, usually because they have a reduced amount of resources and the great majority of them use electric power from batteries. One way to minimize the power consumption of these devices is through of the application of low power consumption techniques. From the various techniques presented in the literature - the intra-task Dynamic Voltage and Frequency Scaling (DVFS) has played an important role. The main aim of DVFS is to allow each task to manage the minimum resources necessary for tasks execution, this way reducing the processor power consumption and, at the same time, respecting the task deadlines when considered a real-time system context. Therefore, this paper aims to apply a systematic literature review with the goal of identifying and presenting the main methods using the intra-task DVFS technique, applied in the context of real-time systems to reduce energy consumption on the processor. Finally, this work will show the advantages and disadvantages of each cataloged methodology.

==> Capitulos/apendice_base_de_dados_backup.tex <==
\section{Base de Dados da Revisão Sistemática}
\label{section:Apendice_Base_Dados_Revisao_Sistematica}

Todas as informações coletadas e catalogadas após a execução do 2\textordmasculine filtro foram tabeladas em ordem cronológica e agrupada de acordo com os critérios de extração de dados definidos na Seção~\ref{subsection:Procedimentos_Extracao_Dados}. As tabelas a seguir mostram todos os dados extraídos de cada uma das 39 publicações selecionadas no 2\textordmasculine filtro.


%**********************************************************
% PUBLICACAO - ID_EXCEL: 257
%**********************************************************
%\newpage
\begin{table}[htp] % h:here; t:top; b:bottom; p:page; default:ht
\centering
\caption{Dados extraído da publicação de \cite{Shin_Kim_2001_a}.}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{|p{3.8cm}|p{16cm}|}
\hline
\multicolumn{1}{|r|}{\textbf{ID}} & Shin\_Kim\_2001\_a \\ \hline
\multicolumn{1}{|r|}{\textbf{Título}} & A profile-based energy-efficient intra-task voltage scheduling algorithm for hard real-time applications \\ \hline
\multicolumn{1}{|r|}{\textbf{Autores}} & Shin D., Kim J. \\ \hline
\multicolumn{1}{|r|}{\textbf{Palavras-chave}} & Algorithms; Decoding; Delay circuits; Energy utilization; Probability; Voltage control; Dynamic voltage scaling; CMOS integrated circuits \\ \hline
\multicolumn{1}{|r|}{\textbf{Fonte da publicação}} & International Symposium on Low Electronics and Design (ISLPED'01) \\ \hline
\multicolumn{1}{|r|}{\textbf{Editora}} & ACM and IEEE \\ \hline
\multicolumn{1}{|r|}{\textbf{Ano da publicação}} & 2001 \\ \hline \hline

\multicolumn{2}{|c|}{\textbf{Resumo da publicação}} \\ \hline
\multicolumn{2}{|p{20cm}|}{Os autores foram os precursores no desenvolvimento de ferramentas para análise do WCET intra-tarefa em aplicações de tempo real. A principal finalidade dos algoritmos da ferramenta eram controlar a velocidade de execução da aplicação baseado nos caminhos de execução de caso médio (em inglês, \textit{Average-Case Execution Path - ACEP}), que são os caminhos mais frequentemente executados. Com essa abordagem os autores conseguiram provar que o algoritmo proposto é mais eficaz na redução do consumo de energia que o algoritmo original intraVS, chamado pelos autores de \textit{(RWEP)-based IntraVS} (em inglês, \textit{Remaining Worst-Case Execution Path-based Intra VS}), onde mesmo utilizando as ACEPs é possível satisfazer as restrições temporais da aplicação de tempo real. Esse método se baseia no perfil de comportamento da aplicação, através da análise dos caminhos de execução mais utilizados (ou \textit{hot paths}), chamado de \textit{(RAEP)-based IntraVS} (em inglês, \textit{Remaining Average-Case Execution Path-based IntraVS}). Sua principal contribuição está na exploração das probabilidades de cada caminho de execução da aplicação e garantir que as restrições temporais sejam respeitadas mesmo executando o pior caso. Os experimentos mostram que o \textit{RAEP-based} é 34\% mais eficiente energeticamente que o \textit{RWEP-based}.} \\ \hline \hline

\multicolumn{1}{|r|}{\textbf{Método(s) utilizados}} & DVFS Intra-Task; Control Flow Graph (CFG); \\ \hline
\multicolumn{1}{|r|}{\textbf{Ferramenta(s)}} & {Os autores utilizaram a ferramenta \textit{Automatic Voltage Scaler} (AVS) [Não disponível para Download]. \newline

Os autores utilizaram o seguinte \textit{benchmark}: \newline
- MPEG-4 \textit{decoder}} \\ \hline \hline

\multicolumn{2}{|c|}{\textbf{Impacto (positivo x negativo)}} \\ \hline
\multicolumn{2}{|p{20cm}|}{O artigo apresentou como ponto positivo uma nova metodologia que explora as probabilidades de cada caminho de execução da aplicação, tomando como base os \textit{hot paths} do caso médio (ACE), e provou que é possível reduzir o consumo de energia e respeitar as restrições temporais de todas as tarefas.. Como ponto negativo, a metodologia não dá suporte a preempções e não mostrou casos de teste para analisar o desempenho da aplicação diante da inserção de muitos pontos de escalonamento de tensão.} \\ \hline \hline

\multicolumn{2}{|c|}{\textbf{Validação do método}} \\ \hline
\multicolumn{2}{|p{20cm}|}{A validação da metodologia ocorreu através do uso de ferramentas e \textit{benchmarks} relatados na literatura. Além disso, compara os resultados experimentais com outros trabalhos de referência na área de baixo consumo de energia.} \\ \hline \hline

\multicolumn{2}{|c|}{\textbf{Limitações do método}} \\ \hline
\multicolumn{2}{|p{20cm}|}{A metodologia não dá suporte a preempções e não mostrou casos de teste para analisar o desempenho da aplicação diante da inserção de muitos pontos de escalonamento de tensão.} \\ \hline \hline

\multicolumn{2}{|c|}{\textbf{Integração de métodos}} \\ \hline
\multicolumn{2}{|p{20cm}|}{Não se aplica} \\ \hline \hline

\multicolumn{2}{|c|}{\textbf{Modo de aplicação do método}} \\ \hline
\multicolumn{2}{|p{20cm}|}{Offline} \\ \hline \hline

\multicolumn{2}{|c|}{\textbf{Perspectivas futuras}} \\ \hline
\multicolumn{2}{|p{20cm}|}{Não identificada} \\ \hline \hline

\multicolumn{2}{|c|}{\textbf{Comentários}} \\ \hline
\multicolumn{2}{|p{20cm}|}{A metodologia proposta não mostra evidências, no artigo, de que fornece suporte para recursos compartilhados e / ou preempções.} \\ \hline
\end{tabular}
}
\end{table}


%**********************************************************
% PUBLICACAO - ID_EXCEL: 256
%**********************************************************
\newpage
\begin{table}[htp] % h:here; t:top; b:bottom; p:page; default:ht
\centering
\caption{Dados extraído da publicação de \cite{Shin_Kim_Lee_2001_a}.}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{|p{3.8cm}|p{16cm}|}
\hline
\multicolumn{1}{|r|}{\textbf{ID}} & Shin\_Kim\_Lee\_2001\_a \\ \hline
\multicolumn{1}{|r|}{\textbf{Título}} & Intra-task voltage scheduling for low-energy hard real-time applications \\ \hline
\multicolumn{1}{|r|}{\textbf{Autores}} & Shin D., Kim J., Lee S. \\ \hline
\multicolumn{1}{|r|}{\textbf{Palavras-chave}} & Dynamic power consumption; Dynamic voltage scaling technique; Intra-task voltage scheduling; Velocity saturation index; Algorithms; Capacitance; CMOS integrated circuits; Computer software; Performance; Portable equipment; Reliability; Threshold voltage; VLSI circuits; Electric power supplies to apparatus \\ \hline
\multicolumn{1}{|r|}{\textbf{Fonte da publicação}} & IEEE Design and Test of Computers \\ \hline
\multicolumn{1}{|r|}{\textbf{Editora}} & IEEE \\ \hline
\multicolumn{1}{|r|}{\textbf{Ano da publicação}} & 2001 \\ \hline \hline

\multicolumn{2}{|c|}{\textbf{Resumo da publicação}} \\ \hline
\multicolumn{2}{|p{20cm}|}{Os autores propõem um novo algoritmo de escalonamento de tensão intra-tarefa que controla a tensão de alimentação do processador durante a execução da tarefa, através da exploração dos tempos de folga. Esse método se baseia na análise do tempo de execução estático e na inserção de códigos, dentro do código fonte da aplicação, para a realização dos chaveamentos de tensões e frequências do processador, de forma que o consumo geral de energia seja reduzido. Esses códigos de chaveamento de tensão são definidos para cada um dos blocos de código selecionados a partir do grafo de fluxo de controle da aplicação (CFG). Dessa forma é possível definir as tensões e frequências para cada bloco de código, aproximando assim o tempo de execução ao deadline da tarefa, sempre respeitando as restrições temporais de todas as tarefas em execução. Neste trabalho os autores introduziram uma nova perspectiva para analisar as CFGs, que consiste em mapear os blocos de código por estruturas condicionais (chamado de \textit{B-types}) e por estruturas de repetição (chamado de \textit{L-types}), dessa forma é mais fácil analisar e predizer os cálculos do WCEC (em inglês, \textit{Worst Case Execution Cycle}) e RWCEC (em inglês, \textit{Remaining Worst Case Execution Cycle}). Todas essas analises foram introduzidas na ferramenta AVS (em inglês, \textit{Automatic Voltage Scaler}), desenvolvida pelos próprios autores. O único ponto negativo no estudo realizado é a falta de métricas para avaliar os reais impactos causados pela inserção de códigos adicionais dentro das aplicações.} \\ \hline \hline

\multicolumn{1}{|r|}{\textbf{Método(s) utilizados}} & DVFS Intra-Task; Control Flow Graph (CFG); \\ \hline
\multicolumn{1}{|r|}{\textbf{Ferramenta(s)}} & {Os autores utilizaram a ferramenta \textit{Automatic Voltage Scaler} (AVS) [Não disponível para Download]. \newline

Os autores utilizaram o seguinte \textit{benchmark}: \newline
- MPEG4 \textit{decoder}} \\ \hline \hline

\multicolumn{2}{|c|}{\textbf{Impacto (positivo x negativo)}} \\ \hline
\multicolumn{2}{|p{20cm}|}{O artigo apresentou como ponto positivo uma nova metodologia para a inserção automática de pontos de escalonamento de tensão, de forma que cada bloco de código extraído da aplicação possa ser executado com valores de tensão e frequência ideais. Como ponto negativo, a metodologia não dá suporte a preempções e não mostrou estudos de caso para avaliar o impacto da inserção de muitos pontos de chaveamento de tensão dentro do código fonte da aplicação.} \\ \hline \hline

\multicolumn{2}{|c|}{\textbf{Validação do método}} \\ \hline
\multicolumn{2}{|p{20cm}|}{A validação da metodologia ocorreu através do uso de ferramentas e \textit{benchmarks} relatados na literatura.} \\ \hline \hline

\multicolumn{2}{|c|}{\textbf{Limitações do método}} \\ \hline
\multicolumn{2}{|p{20cm}|}{A metodologia não dá suporte a preempções e não mostrou estudos de caso para avaliar o impacto da inserção de muitos pontos de chaveamento de tensão dentro do código fonte da aplicação.} \\ \hline \hline

\multicolumn{2}{|c|}{\textbf{Integração de métodos}} \\ \hline
\multicolumn{2}{|p{20cm}|}{Não se aplica} \\ \hline \hline

\multicolumn{2}{|c|}{\textbf{Modo de aplicação do método}} \\ \hline
\multicolumn{2}{|p{20cm}|}{Offline} \\ \hline \hline

\multicolumn{2}{|c|}{\textbf{Perspectivas futuras}} \\ \hline
\multicolumn{2}{|p{20cm}|}{Os autores pretendem realizar uma comparação quantitativa entre as abordagens intra-tarefa e inter-tarefa.} \\ \hline \hline

\multicolumn{2}{|c|}{\textbf{Comentários}} \\ \hline
\multicolumn{2}{|p{20cm}|}{A metodologia proposta não mostra evidências, no artigo, de que fornece suporte para recursos compartilhados e / ou preempções.} \\ \hline
\end{tabular}
}
\end{table}


%**********************************************************
% PUBLICACAO - ID_EXCEL: 255
%**********************************************************
\newpage
\begin{table}[htp] % h:here; t:top; b:bottom; p:page; default:ht
\centering
\caption{Dados extraído da publicação de \cite{Shin_Kim_Lee_2001_b}.}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{|p{3.8cm}|p{16cm}|}
\hline
\multicolumn{1}{|r|}{\textbf{ID}} & Shin\_Kim\_Lee\_2001\_b \\ \hline
\multicolumn{1}{|r|}{\textbf{Título}} & Low-energy intra-task voltage scheduling using static timing analysis \\ \hline
\multicolumn{1}{|r|}{\textbf{Autores}} & Shin D., Kim J., Lee S. \\ \hline
\multicolumn{1}{|r|}{\textbf{Palavras-chave}} & Algorithms; Computer aided software engineering; Image coding; VLSI circuits; Voltage scheduling; Real time systems \\ \hline
\multicolumn{1}{|r|}{\textbf{Fonte da publicação}} & 38th Design Automation Conference; Las Vegas, NV; United States; \\ \hline
\multicolumn{1}{|r|}{\textbf{Editora}} & IEEE \\ \hline
\multicolumn{1}{|r|}{\textbf{Ano da publicação}} & 2001 \\ \hline \hline

\multicolumn{2}{|c|}{\textbf{Resumo da publicação}} \\ \hline
\multicolumn{2}{|p{20cm}|}{Os autores propõem uma nova metodologia para analise do WCET (em inglês, \textit{Worst Case Execution Time}) em aplicações de tempo real e tomaram com base o trabalho de \cite{Shin_Kim_Lee_2001_a}. Essa análise é feita em tempo de compilação, de modo \textit{offline}, utilizando o grafo de fluxo de controle da aplicação, onde o cálculo do WCET é feita para cada nó da CFG, enquanto que no trabalho anterior dos mesmos autores a estimativa do WCET era feita tendo como base o programa inteiro.} \\ \hline \hline

\multicolumn{1}{|r|}{\textbf{Método(s) utilizados}} & DVFS Intra-Task; Control Flow Graph (CFG); \\ \hline
\multicolumn{1}{|r|}{\textbf{Ferramenta(s)}} & {Os autores utilizaram a ferramenta \textit{Automatic Voltage Scaler} (AVS) [Ferramenta não localizada] \newline

Os autores utilizaram o seguinte \textit{benchmark}: \newline
- MPEG-4 \textit{encoder e decoder}} \\ \hline \hline

\multicolumn{2}{|c|}{\textbf{Impacto (positivo x negativo)}} \\ \hline
\multicolumn{2}{|p{20cm}|}{O artigo apresentou como ponto positivo uma nova metodologia para realizar análises estáticas dos tempos de execução da aplicação, visando mapear os tempos de folga e, principalmente, identificar as tensões e frequências ideais que devem ser aplicadas no processador para que a tarefa termine de executar o mais próximo possível do seu deadline, economizando energia. Como ponto negativo, a metodologia não dá suporte a preempções.} \\ \hline \hline

\multicolumn{2}{|c|}{\textbf{Validação do método}} \\ \hline
\multicolumn{2}{|p{20cm}|}{A validação da metodologia ocorreu através do uso de ferramentas e \textit{benchmarks} relatados na literatura.} \\ \hline \hline

\multicolumn{2}{|c|}{\textbf{Limitações do método}} \\ \hline
\multicolumn{2}{|p{20cm}|}{A metodologia não dá suporte a preempções.} \\ \hline \hline

\multicolumn{2}{|c|}{\textbf{Integração de métodos}} \\ \hline
\multicolumn{2}{|p{20cm}|}{Não se aplica} \\ \hline \hline

\multicolumn{2}{|c|}{\textbf{Modo de aplicação do método}} \\ \hline
\multicolumn{2}{|p{20cm}|}{Offline} \\ \hline \hline

\multicolumn{2}{|c|}{\textbf{Perspectivas futuras}} \\ \hline
\multicolumn{2}{|p{20cm}|}{O autor pretende incluir no método proposto outras informações, em tempo de execução, para melhor o algoritmo de escalonamento e a redução do consumo de energia do processador.} \\ \hline \hline

\multicolumn{2}{|c|}{\textbf{Comentários}} \\ \hline
\multicolumn{2}{|p{20cm}|}{A metodologia proposta não mostra evidências, no artigo, de que fornece suporte para recursos compartilhados e / ou preempções.} \\ \hline
\end{tabular}
}
\end{table}


%**********************************************************
% PUBLICACAO - ID_EXCEL: 248
%**********************************************************
\newpage
\begin{table}[htp] % h:here; t:top; b:bottom; p:page; default:ht
\centering
\caption{Dados extraído da publicação de \cite{Lee_Yoo_Choi_2002_a}.}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{|p{3.8cm}|p{16cm}|}
\hline
\multicolumn{1}{|r|}{\textbf{ID}} & Lee\_Yoo\_Choi\_2002\_a \\ \hline
\multicolumn{1}{|r|}{\textbf{Título}} & An intra-task dynamic voltage scaling method for SoC design with hierarchical FSM and synchronous dataflow model \\ \hline
\multicolumn{1}{|r|}{\textbf{Autores}} & Lee S., Yoo S., Choi K. \\ \hline
\multicolumn{1}{|r|}{\textbf{Palavras-chave}} & Dynamic voltage scaling; Finite state machine; Formal model; Low power; Synchronous dataflow; Variable supply voltage \\ \hline
\multicolumn{1}{|r|}{\textbf{Fonte da publicação}} & Proceedings of the 2002 International Symposium on Low Power Electronics and Design; Monterey, CA;  \\ \hline
\multicolumn{1}{|r|}{\textbf{Editora}} & ACM \\ \hline
\multicolumn{1}{|r|}{\textbf{Ano da publicação}} & 2002 \\ \hline \hline

\multicolumn{2}{|c|}{\textbf{Resumo da publicação}} \\ \hline
\multicolumn{2}{|p{20cm}|}{Os autores propõem um método de escalonamento de tensão para o projeto de SoCs (em inglês, \textit{System on a Chips}) com hierarquia FSM (em inglês, \textit{Finite State Machine}) e modelo de dados síncrono. Essa técnica foi chamada de modelo HFSM-SDF (em inglês, \textit{Hierarchical FSM and Synchronous Dataflow Model}). Essa metodologia calcula o caminho de execução da aplicação em tempo de execução e utiliza muitos dos conceitos definidos por \cite{Shin_Kim_Lee_2001_a}, para calcular a carga de trabalho restante das tarefas de tempo real e assim aplicar sobre o processador as tensões e frequências ideais para que o consumo de energia seja o menor possível.} \\ \hline \hline

\multicolumn{1}{|r|}{\textbf{Método(s) utilizados}} & DVFS Intra-Task; Control Flow Graph (CFG); \\ \hline
\multicolumn{1}{|r|}{\textbf{Ferramenta(s)}} & {Os autores utilizaram a ferramenta ARMulator [Disponível em: \href{http://x-y-z.github.io/armulator/}{http://x-y-z.github.io/armulator/}]. \newline

Os autores utilizaram o seguinte \textit{benchmark}: \newline
- MPEG-4 \textit{natural video decoder} [Disponível em: \href{http://www.m4if.org/}{http://www.m4if.org/}].} \\ \hline \hline

\multicolumn{2}{|c|}{\textbf{Impacto (positivo x negativo)}} \\ \hline
\multicolumn{2}{|p{20cm}|}{O artigo apresentou como ponto positivo uma nova metodologia online para calcular a carga de trabalho restante da aplicação e as tensões e frequências ideais que devem ser aplicadas no processador. Como ponto negativo, a metodologia não leva em consideração múltiplas tarefas em execução.} \\ \hline \hline

\multicolumn{2}{|c|}{\textbf{Validação do método}} \\ \hline
\multicolumn{2}{|p{20cm}|}{A validação da metodologia ocorreu através do uso de ferramentas e \textit{benchmarks} relatados na literatura.} \\ \hline \hline

\multicolumn{2}{|c|}{\textbf{Limitações do método}} \\ \hline
\multicolumn{2}{|p{20cm}|}{A metodologia não leva em consideração um ambiente com múltiplas tarefas em execução.} \\ \hline \hline

\multicolumn{2}{|c|}{\textbf{Integração de métodos}} \\ \hline
\multicolumn{2}{|p{20cm}|}{Não se aplica} \\ \hline \hline

\multicolumn{2}{|c|}{\textbf{Modo de aplicação do método}} \\ \hline
\multicolumn{2}{|p{20cm}|}{Híbrida} \\ \hline \hline

\multicolumn{2}{|c|}{\textbf{Perspectivas futuras}} \\ \hline
\multicolumn{2}{|p{20cm}|}{Extender o método proposto para um ambiente com multi-tarefas e dar suporte a preempções.} \\ \hline \hline

\multicolumn{2}{|c|}{\textbf{Comentários}} \\ \hline
\multicolumn{2}{|p{20cm}|}{A metodologia proposta não mostra evidências, no artigo, de que fornece suporte para recursos compartilhados e / ou preempções.} \\ \hline
\end{tabular}
}
\end{table}


%**********************************************************
% PUBLICACAO - ID_EXCEL: 238
%**********************************************************
\newpage
\begin{table}[htp] % h:here; t:top; b:bottom; p:page; default:ht
\centering
\caption{Dados extraído da publicação de \cite{Aboughazaleh_2003_a}.}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{|p{3.8cm}|p{16cm}|}
\hline
\multicolumn{1}{|r|}{\textbf{ID}} & Aboughazaleh\_2003\_a \\ \hline
\multicolumn{1}{|r|}{\textbf{Título}} & Energy management for real-time embedded applications with compiler support \\ \hline
\multicolumn{1}{|r|}{\textbf{Autores}} & AbouGhazaleh N., Childers B., Mosse D., Melhem R., Craven M. \\ \hline
\multicolumn{1}{|r|}{\textbf{Palavras-chave}} & Dynamic voltage scaling; Power management; Real-time \\ \hline
\multicolumn{1}{|r|}{\textbf{Fonte da publicação}} & Proceedings of the ACM SIGPLAN Conference on Languages, Compilers, and Tools for Embedded Systems (LCTES) \\ \hline
\multicolumn{1}{|r|}{\textbf{Editora}} & ACM \\ \hline
\multicolumn{1}{|r|}{\textbf{Ano da publicação}} & 2003 \\ \hline \hline

\multicolumn{2}{|c|}{\textbf{Resumo da publicação}} \\ \hline
\multicolumn{2}{|p{20cm}|}{Os autores propõem uma técnica que explora as variações dos tempos de execução em diferentes caminhos de execução da aplicação. Esta é uma abordagem híbrida que depende do compilador e do sistema operacional para melhor gerenciar o desempenho e a redução do consumo de energia do processador. O compilador então insere os chamados PMHs (em inglês, \textit{Power Management Hints}), que são trechos de código responsáveis por fornecer e coletar informações em tempo de execução da aplicação para o sistema operacional, além de estimar o desempenho da aplicação no pior caso. Dessa forma, o sistema operacional invoca os PMPs (em inglês, \textit{Power Management Points}) para realizar o chaveamento de tensão e frequência do processador com base nas informações passadas pelos PMHs.} \\ \hline \hline

\multicolumn{1}{|r|}{\textbf{Método(s) utilizados}} & DVFS Intra-Task; Control Flow Graph (CFG); \\ \hline
\multicolumn{1}{|r|}{\textbf{Ferramenta(s)}} & {Os autores utilizaram a ferramenta Simplescalar Micro-architecture Toolkit [Disponível em: \href{http://www.simplescalar.com/}{http://www.simplescalar.com/}]. \newline

Os autores utilizaram os seguintes \textit{benchmarks}: \newline
- MPEG-2 \textit{decoder} [Disponível em: \href{http://www.mpeg.org/}{http://www.mpeg.org/}]. \newline
- \textit{Automatic Target Recognition} (ATR) \textit{Application}.} \\ \hline \hline

\multicolumn{2}{|c|}{\textbf{Impacto (positivo x negativo)}} \\ \hline
\multicolumn{2}{|p{20cm}|}{O artigo apresentou como ponto positivo uma nova metodologia que visa integrar o compilador e o sistema operacional para trabalharem em conjunto na redução do consumo de energia do processador. Como ponto negativo, a metodologia foi modelada apenas para tarefas não preemptivas e durante a etapa de experimentações constatou-se que o desempenho da aplicação pode ser prejudicado dependendo da quantidade de instruções inseridas pelo compilador.} \\ \hline \hline

\multicolumn{2}{|c|}{\textbf{Validação do método}} \\ \hline
\multicolumn{2}{|p{20cm}|}{A validação da metodologia ocorreu através do uso de ferramentas e \textit{benchmarks} relatados na literatura. Além disso, compara os resultados experimentais com outros trabalhos de referência na área de baixo consumo de energia.} \\ \hline \hline

\multicolumn{2}{|c|}{\textbf{Limitações do método}} \\ \hline
\multicolumn{2}{|p{20cm}|}{A metodologia não dá suporte a preempções e pode prejudicar o desempenho das aplicações dependendo da quantidade de instruções inseridas pelo compilador.} \\ \hline \hline

\multicolumn{2}{|c|}{\textbf{Integração de métodos}} \\ \hline
\multicolumn{2}{|p{20cm}|}{Não se aplica} \\ \hline \hline

\multicolumn{2}{|c|}{\textbf{Modo de aplicação do método}} \\ \hline
\multicolumn{2}{|p{20cm}|}{Híbrida} \\ \hline \hline

\multicolumn{2}{|c|}{\textbf{Perspectivas futuras}} \\ \hline
\multicolumn{2}{|p{20cm}|}{O autor pretende incluir no seu método a extração de informações inter-tarefas.} \\ \hline \hline

\multicolumn{2}{|c|}{\textbf{Comentários}} \\ \hline
\multicolumn{2}{|p{20cm}|}{A metodologia proposta não mostra evidências, no artigo, de que fornece suporte para recursos compartilhados e / ou preempções.} \\ \hline
\end{tabular}
}
\end{table}


%**********************************************************
% PUBLICACAO - ID_EXCEL: 234
%**********************************************************
%\newpage
\begin{table}[htp] % h:here; t:top; b:bottom; p:page; default:ht
\centering
\caption{Dados extraído da publicação de \cite{Buss_Givargis_Dutt_2003_a}.}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{|p{3.8cm}|p{16cm}|}
\hline
\multicolumn{1}{|r|}{\textbf{ID}} & Buss\_Givargis\_Dutt\_2003\_a \\ \hline
\multicolumn{1}{|r|}{\textbf{Título}} & Exploring efficient operating points for voltage scaled embedded processor cores \\ \hline
\multicolumn{1}{|r|}{\textbf{Autores}} & Buss M., Givargis T., Dutt N. \\ \hline
\multicolumn{1}{|r|}{\textbf{Palavras-chave}} & Algorithms; CMOS integrated circuits; Electric potential; Multimedia systems; Personal digital assistants; Reduced instruction set computing; Scheduling; Dynamic voltage scaled processors; Instruction-set tailoring; Register file sizing; Voltage scaled embedded processor cores; Embedded systems \\ \hline
\multicolumn{1}{|r|}{\textbf{Fonte da publicação}} & 24th IEEE International Real-Time Systems Symposium RTSS 2003 \\ \hline
\multicolumn{1}{|r|}{\textbf{Editora}} & ACM and IEEE \\ \hline
\multicolumn{1}{|r|}{\textbf{Ano da publicação}} & 2003 \\ \hline \hline

\multicolumn{2}{|c|}{\textbf{Resumo da publicação}} \\ \hline
\multicolumn{2}{|p{20cm}|}{Os autores propõem a exploração e seleção de potenciais pontos de escalonamento de tensão que possam atuar na diminuição eficiente do consumo de energia em aplicações de tempo real não críticos. A problemática desse método está em selecionar esses pontos de controle para atuar em conjunto com a técnica DVS intra-tarefa, proporcionando uma redução do consumo de energia do processador. Esse método se baseia basicamente em três passos, são eles: (1) fazer a análise estática da aplicação e atribuir um fator de desaceleração ideal para cada bloco; (2) computar as frequências de operação com base na análise da aplicação inteira; (3) reatribuir os fatores de aceleração para cada bloco, com base nas frequências de operação válidas e computadas no passo 2. Essa abordagem é muito semelhante a técnica dos coreanos \citep{Shin_Kim_Lee_2001_a}, onde a principal diferença esta na metodologia de definição dos fatores de desaceleração.} \\ \hline \hline

\multicolumn{1}{|r|}{\textbf{Método(s) utilizados}} & DVFS Intra-Task; Control Flow Graph (CFG); \\ \hline
\multicolumn{1}{|r|}{\textbf{Ferramenta(s)}} & {Os autores utilizaram a ferramenta WARTS / EEL (\textit{Executable Editing Library}) [Disponível em: \href{http://pages.cs.wisc.edu/~larus/eel.html}{http://pages.cs.wisc.edu/$\sim$larus/eel.html}]. \newline

Os autores utilizaram os seguintes \textit{benchmarks}: \newline
- MiBench [Disponível em: \href{http://www.eecs.umich.edu/mibench/}{http://www.eecs.umich.edu/mibench/}] \newline
- Powerstone \newline
- MediaBench [Disponível em: \href{http://cares.icsl.ucla.edu/MediaBench}{http://cares.icsl.ucla.edu/MediaBench}] \newline
- lame (MP3 \textit{encoding engine}) \newline
- jpeg (\textit{Image compression and decompression}) \newline
- compress (\textit{Data compression tool}) \newline
- engine (\textit{Engine controller}) \newline
- mpeg (\textit{Video encoder}) \newline
- madplay (MPEG \textit{audio decoder}) \newline
- tiff2ps (Tiff \textit{to postscript conversion}) \newline
- gsm (\textit{Speech transcoding}) \newline
- basicmath (\textit{Basic math operations}) \newline
- adpcm (\textit{Voice encoder}) \newline
- dijkstra (\textit{Shortest path algorithm})} \\ \hline \hline

\multicolumn{2}{|c|}{\textbf{Impacto (positivo x negativo)}} \\ \hline
\multicolumn{2}{|p{20cm}|}{O artigo apresentou como ponto positivo uma nova metodologia para realizar a analise e classificação de blocos de código quanto ao seu fator de desaceleração, que permite ter um controle mais refinado sobre as tensões e frequências ideais que devem ser aplicadas sobre o processador. Como ponto negativo, a metodologia não deixa claro se dar suporte há algumas estruturas de dados como \textit{loops} ocultos e recursões.} \\ \hline \hline

\multicolumn{2}{|c|}{\textbf{Validação do método}} \\ \hline
\multicolumn{2}{|p{20cm}|}{A validação da metodologia ocorreu através do uso de ferramentas e \textit{benchmarks} relatados na literatura.} \\ \hline \hline

\multicolumn{2}{|c|}{\textbf{Limitações do método}} \\ \hline
\multicolumn{2}{|p{20cm}|}{A metodologia não deixa claro se dar suporte há algumas estruturas de dados como \textit{loops} ocultos e recursões.} \\ \hline \hline

\multicolumn{2}{|c|}{\textbf{Integração de métodos}} \\ \hline
\multicolumn{2}{|p{20cm}|}{Não se aplica} \\ \hline \hline

\multicolumn{2}{|c|}{\textbf{Modo de aplicação do método}} \\ \hline
\multicolumn{2}{|p{20cm}|}{Offline} \\ \hline \hline

\multicolumn{2}{|c|}{\textbf{Perspectivas futuras}} \\ \hline
\multicolumn{2}{|p{20cm}|}{Os autores pretendem incluir os custos de tempo e energia para melhorar a eficiência do seu método, tornando assim a metodologia mais realista e preciso.} \\ \hline \hline

\multicolumn{2}{|c|}{\textbf{Comentários}} \\ \hline
\multicolumn{2}{|p{20cm}|}{A metodologia proposta não mostra evidências, no artigo, de que fornece suporte para recursos compartilhados e / ou preempções.} \\ \hline
\end{tabular}
}
\end{table}


%**********************************************************
% PUBLICACAO - ID_EXCEL: 232
%**********************************************************
\newpage
\begin{table}[htp] % h:here; t:top; b:bottom; p:page; default:ht
\centering
\caption{Dados extraído da publicação de \cite{Aboughazaleh_2003_b}.}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{|p{3.8cm}|p{16cm}|}
\hline
\multicolumn{1}{|r|}{\textbf{ID}} & Aboughazaleh\_2003\_b \\ \hline
\multicolumn{1}{|r|}{\textbf{Título}} & Collaborative operating system and compiler power management for real-time applications \\ \hline
\multicolumn{1}{|r|}{\textbf{Autores}} & Aboughazaleh N., Mosse D., Childers B., Melhem R., Craven M. \\ \hline
\multicolumn{1}{|r|}{\textbf{Palavras-chave}} & Collaborative approach; Dynamic power consumption; Dynamic voltage scaling; Embedded application; Power management points; Real-time application; Reduce energy consumption; Temporal information \\ \hline
\multicolumn{1}{|r|}{\textbf{Fonte da publicação}} & 9th IEEE Real-Time and Embedded Technology and Applications Symposium, RTAS 2003 \\ \hline
\multicolumn{1}{|r|}{\textbf{Editora}} & IEEE \\ \hline
\multicolumn{1}{|r|}{\textbf{Ano da publicação}} & 2003 \\ \hline \hline

\multicolumn{2}{|c|}{\textbf{Resumo da publicação}} \\ \hline
\multicolumn{2}{|p{20cm}|}{Os autores tomaram como base o trabalho de \cite{Aboughazaleh_2003_a}, onde o foco principal da metodologia passou a ser a colaboração entre o compilador e o sistema operacional. O principal contribuição em relação ao trabalho anterior está no sistema operacional, que passa a monitorar periodicamente os chaveamentos de tensões e frequências do processador baseado nas informações providas pelos \textit{PMHs}.} \\ \hline \hline

\multicolumn{1}{|r|}{\textbf{Método(s) utilizados}} & DVFS Intra-Task; Control Flow Graph (CFG); \\ \hline
\multicolumn{1}{|r|}{\textbf{Ferramenta(s)}} & {Os autores utilizaram a ferramenta Sim-Outorder Simulator from SimpleScalar [Disponível em: \href{http://www.simplescalar.com/}{http://www.simplescalar.com/}]. \newline

Os autores utilizaram os seguintes \textit{benchmarks}: \newline
- MPEG2 \textit{decoder} [Disponível em: \href{http://www.mpeg.org/}{http://www.mpeg.org/}] \newline
- \textit{Automated Target Recognition} (ATR)} \\ \hline \hline

\multicolumn{2}{|c|}{\textbf{Impacto (positivo x negativo)}} \\ \hline
\multicolumn{2}{|p{20cm}|}{O artigo apresentou como ponto positivo uma metodologia cuja finalidade é criar um canal de comunicação entre o compilador e o sistema operacional, permitindo que ambos possam trabalhar em conjunto para a diminuição do consumo de energia do processador. Além disso, a metodologia utilizada dá suporte a preempções. Como ponto negativo, a metodologia insere uma quantidade excessiva de \textit{overheads} dentro da aplicação.} \\ \hline \hline

\multicolumn{2}{|c|}{\textbf{Validação do método}} \\ \hline
\multicolumn{2}{|p{20cm}|}{A validação da metodologia ocorreu através do uso de ferramentas e \textit{benchmarks} relatados na literatura. Além disso, compara os resultados experimentais com outros trabalhos de referência na área de baixo consumo de energia.} \\ \hline \hline

\multicolumn{2}{|c|}{\textbf{Limitações do método}} \\ \hline
\multicolumn{2}{|p{20cm}|}{A metodologia insere uma quantidade excessiva de \textit{overheads} dentro da aplicação.} \\ \hline \hline

\multicolumn{2}{|c|}{\textbf{Integração de métodos}} \\ \hline
\multicolumn{2}{|p{20cm}|}{Não se aplica} \\ \hline \hline

\multicolumn{2}{|c|}{\textbf{Modo de aplicação do método}} \\ \hline
\multicolumn{2}{|p{20cm}|}{Híbrida} \\ \hline \hline

\multicolumn{2}{|c|}{\textbf{Perspectivas futuras}} \\ \hline
\multicolumn{2}{|p{20cm}|}{Não identificada} \\ \hline \hline

\multicolumn{2}{|c|}{\textbf{Comentários}} \\ \hline
\multicolumn{2}{|p{20cm}|}{A metodologia dá suporte a preempções, através da chamada de interrupções do sistema operacional para adaptar as tensões e frequências do processador. Quanto aos recursos compartilhados, a metodologia proposta não dá suporte.} \\ \hline
\end{tabular}
}
\end{table}


%**********************************************************
% PUBLICACAO - ID_EXCEL: 225
%**********************************************************
\newpage
\begin{table}[htp] % h:here; t:top; b:bottom; p:page; default:ht
\centering
\caption{Dados extraído da publicação de \cite{Seo_Kim_Chung_2004_a}.}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{|p{3.8cm}|p{16cm}|}
\hline
\multicolumn{1}{|r|}{\textbf{ID}} & Seo\_Kim\_Chung\_2004\_a \\ \hline
\multicolumn{1}{|r|}{\textbf{Título}} & Profile-based optimal intra-task voltage scheduling for hard real-time applications \\ \hline
\multicolumn{1}{|r|}{\textbf{Autores}} & Seo J., Kim T., Chung K.-S. \\ \hline
\multicolumn{1}{|r|}{\textbf{Palavras-chave}} & DVS; Intra-task voltage scheduling; Low energy design \\ \hline
\multicolumn{1}{|r|}{\textbf{Fonte da publicação}} & DAC '04 Proceedings of the 41st annual Design Automation Conference \\ \hline
\multicolumn{1}{|r|}{\textbf{Editora}} & ACM and IEEE \\ \hline
\multicolumn{1}{|r|}{\textbf{Ano da publicação}} & 2004 \\ \hline \hline

\multicolumn{2}{|c|}{\textbf{Resumo da publicação}} \\ \hline
\multicolumn{2}{|p{20cm}|}{Os autores propõem uma metodologia baseada no perfil de execução da tarefa, onde os níveis de tensão são definidos para cada bloco de código. Esse método tem como objetivo gerenciar melhor os \textit{overheads} de transição, que são totalmente ou parcialmente ignorados nos outros trabalhos presentes na literatura, e obter melhores níveis de redução do consumo de energia do processador. Essa técnica é chamada de ``ROEP-\textit{based technique}'' (ROEP - \textit{Remaining Optimal-Case Execution Path}), que é uma melhoria da metodologia \textit{RAEP-based} proposta por \citep{Shin_Kim_2001_a}, cujo principal foco está relacionado com desperdícios de energia, com as trocas excessivas de tensão e frequência do processador e com a diminuição dos \textit{overheads} inseridos dentro das aplicações. Seguindo a escala cronológica dos trabalhos catalogados nesta revisão sistemática, esta foi uma das primeiras abordagens a otimizar estes parâmetros.} \\ \hline \hline

\multicolumn{1}{|r|}{\textbf{Método(s) utilizados}} & DVFS Intra-Task; Control Flow Graph (CFG); \\ \hline
\multicolumn{1}{|r|}{\textbf{Ferramenta(s)}} & {Os autores não especificaram nenhuma ferramenta para a realização dos experimentos, mas relataram o uso dos seguintes \textit{benchmarks}: amotsa, dawson, gcf, gser, gsimp, hypser, igray, realft, rtnewt, trsec, sncndn e trapzd (OBS.: estes são \textit{benchmarks} retirados do livro "\textit{Numerical Recipes in C}").} \\ \hline \hline

\multicolumn{2}{|c|}{\textbf{Impacto (positivo x negativo)}} \\ \hline
\multicolumn{2}{|p{20cm}|}{O artigo apresentou como ponto positivo uma metodologia para gerenciar melhor os \textit{overheads} de transição, que são totalmente ou parcialmente ignorados nos trabalhos presentes na literatura. Como ponto negativo, a metodologia não deixa claro se dar suporte há alguns tipos de estruturas como \textit{loops} ocultos e recursões.} \\ \hline \hline

\multicolumn{2}{|c|}{\textbf{Validação do método}} \\ \hline
\multicolumn{2}{|p{20cm}|}{A validação da metodologia ocorreu através do uso de \textit{benchmarks} relatados na literatura. Além disso, compara os resultados experimentais com outros trabalhos de referência na área de baixo consumo de energia.} \\ \hline \hline

\multicolumn{2}{|c|}{\textbf{Limitações do método}} \\ \hline
\multicolumn{2}{|p{20cm}|}{A metodologia não deixa claro se dar suporte há alguns tipos de estruturas como \textit{loops} ocultos e recursões.} \\ \hline \hline

\multicolumn{2}{|c|}{\textbf{Integração de métodos}} \\ \hline
\multicolumn{2}{|p{20cm}|}{Não se aplica} \\ \hline \hline

\multicolumn{2}{|c|}{\textbf{Modo de aplicação do método}} \\ \hline
\multicolumn{2}{|p{20cm}|}{Offline} \\ \hline \hline

\multicolumn{2}{|c|}{\textbf{Perspectivas futuras}} \\ \hline
\multicolumn{2}{|p{20cm}|}{Os autores pretendem verificar os impactos da metodologia proposta quando aplicado em um contexto de escalonamento inter-tarefas.} \\ \hline \hline

\multicolumn{2}{|c|}{\textbf{Comentários}} \\ \hline
\multicolumn{2}{|p{20cm}|}{A metodologia proposta não mostra evidências, no artigo, de que fornece suporte para recursos compartilhados e / ou preempções.} \\ \hline
\end{tabular}
}
\end{table}


%**********************************************************
% PUBLICACAO - ID_EXCEL: 204
%**********************************************************
\newpage
\begin{table}[htp] % h:here; t:top; b:bottom; p:page; default:ht
\centering
\caption{Dados extraído da publicação de \cite{Shin_Kim_2005_a}.}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{|p{3.8cm}|p{16cm}|}
\hline
\multicolumn{1}{|r|}{\textbf{ID}} & Shin\_Kim\_2005\_a \\ \hline
\multicolumn{1}{|r|}{\textbf{Título}} & Intra-task voltage scheduling on DVS-enabled hard real-time systems \\ \hline
\multicolumn{1}{|r|}{\textbf{Autores}} & Shin D., Kim J. \\ \hline
\multicolumn{1}{|r|}{\textbf{Palavras-chave}} & Dynamic voltage scaling; Low-power design; Power management; Real-time systems; Variable-voltage processor \\ \hline
\multicolumn{1}{|r|}{\textbf{Fonte da publicação}} & IEEE Transactions on Computer-Aided Design of Integrated Circuits and Systems \\ \hline
\multicolumn{1}{|r|}{\textbf{Editora}} & IEEE \\ \hline
\multicolumn{1}{|r|}{\textbf{Ano da publicação}} & 2005 \\ \hline \hline

\multicolumn{2}{|c|}{\textbf{Resumo da publicação}} \\ \hline
\multicolumn{2}{|p{20cm}|}{Os autores melhoraram a eficiência do método \textit{RAEP-based} proposto por eles mesmo em \cite{Shin_Kim_2001_a}. Nesta nova abordagem, a principal diferença está nas otimizações de \textit{overheads} para a realização das transições de tensão, que antes era feita de forma \textit{offline} e agora o método de atribuição de tensões passou a ser \textit{online} e mais eficiente. Os autores utilizaram os mesmos casos de teste para realização dos experimentos e fizeram alterações na ferramenta AVS para adaptá-la a nova abordagem. Um fato interessante a ser relatado é que os autores começaram a introduzir o conceito de ciclos salvos ou ciclos economizados (em inglês, \textit{Saved Cycles ou $C_{saved}$}), ou seja, são trechos de código que deixaram de ser executados dentro da aplicação. Esse conceito será melhor amadurecida em \cite{Shin_Kim_2005_b}.} \\ \hline \hline

\multicolumn{1}{|r|}{\textbf{Método(s) utilizados}} & DVFS Intra-Task; Control Flow Graph (CFG); \\ \hline
\multicolumn{1}{|r|}{\textbf{Ferramenta(s)}} & {Os autores utilizaram a ferramenta AVS (\textit{Automatic Voltage Scaler} - Não disponível para download) e o MPEG-4 \textit{enconder / decoder} como \textit{benchmarks}.} \\ \hline \hline

\multicolumn{2}{|c|}{\textbf{Impacto (positivo x negativo)}} \\ \hline
\multicolumn{2}{|p{20cm}|}{O artigo apresentou como ponto positivo uma metodologia que analisa e cria perfis de consumo de energia baseados nos caminhos de execução da aplicação, procurando minimizar os \textit{overheads} introduzidos no código fonte da aplicação. Como ponto negativo, a metodologia não deixa claro se dar suporte a recursões e \textit{loops} ocultos.} \\ \hline \hline

\multicolumn{2}{|c|}{\textbf{Validação do método}} \\ \hline
\multicolumn{2}{|p{20cm}|}{A validação da metodologia ocorreu através do uso de ferramenta e \textit{benchmarks} relatados na literatura. Além disso, compara os resultados experimentais com outros trabalhos de referência na área de baixo consumo de energia.} \\ \hline \hline

\multicolumn{2}{|c|}{\textbf{Limitações do método}} \\ \hline
\multicolumn{2}{|p{20cm}|}{A metodologia não deixa claro se dar suporte a alguns tipos de estruturas como: \textit{loops} ocultos e recursões.} \\ \hline \hline

\multicolumn{2}{|c|}{\textbf{Integração de métodos}} \\ \hline
\multicolumn{2}{|p{20cm}|}{Não se aplica} \\ \hline \hline

\multicolumn{2}{|c|}{\textbf{Modo de aplicação do método}} \\ \hline
\multicolumn{2}{|p{20cm}|}{Híbrida} \\ \hline \hline

\multicolumn{2}{|c|}{\textbf{Perspectivas futuras}} \\ \hline
\multicolumn{2}{|p{20cm}|}{O autor pretende incluir informações em tempo de execução, como por exemplo \textit{cache hit} e \textit{miss}, para melhorar a eficiência energética do método proposto.} \\ \hline \hline

\multicolumn{2}{|c|}{\textbf{Comentários}} \\ \hline
\multicolumn{2}{|p{20cm}|}{A metodologia proposta não mostra evidências, no artigo, de que fornece suporte para recursos compartilhados e / ou preempções.} \\ \hline
\end{tabular}
}
\end{table}


%**********************************************************
% PUBLICACAO - ID_EXCEL: 199
%**********************************************************
\newpage
\begin{table}[htp] % h:here; t:top; b:bottom; p:page; default:ht
\centering
\caption{Dados extraído da publicação de \cite{Yi_Yang_Chen_2005_a}.}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{|p{3.8cm}|p{16cm}|}
\hline
\multicolumn{1}{|r|}{\textbf{ID}} & Yi\_Yang\_Chen\_2005\_a \\ \hline
\multicolumn{1}{|r|}{\textbf{Título}} & The optimal profile-guided greedy dynamic voltage scaling in real-time applications \\ \hline
\multicolumn{1}{|r|}{\textbf{Autores}} & Yi H., Yang X., Chen J. \\ \hline
\multicolumn{1}{|r|}{\textbf{Palavras-chave}} & Computer simulation; Energy utilization; Frequencies; Mathematical models; Program compilers; Real time systems; Scheduling; Dock frequency; Dynamic voltage scaling (DVS); Optimal real-time voltage scheduling; Voltage adjustment; Voltage measurement \\ \hline
\multicolumn{1}{|r|}{\textbf{Fonte da publicação}} & ICESS'05 Proceedings of the Second international conference on Embedded Software and Systems \\ \hline
\multicolumn{1}{|r|}{\textbf{Editora}} & Springer \\ \hline
\multicolumn{1}{|r|}{\textbf{Ano da publicação}} & 2005 \\ \hline \hline

\multicolumn{2}{|c|}{\textbf{Resumo da publicação}} \\ \hline
\multicolumn{2}{|p{20cm}|}{Os autores propõem um modelo analítico de escalonamento dinâmico de tensão "ganancioso", cujo o objetivo é encontrar as tensões ideais para as aplicações de tempo real, através da análise dos casos de execução mais frequentes, ou também chamados de \textit{Hot Path}, referenciados em \cite{Shin_Kim_2001_a}. Essas análises visam identificar os tempos de folga distribuídos pela aplicação e, em seguida, repassa os ganhos obtidos para o processador, minimizando o consumo do energia. Esse método foi chamado de OPTDVS (em inglês, \textit{Optimal Dinamic Voltage Scheduling}). Em outras palavras, esse método é um mecanismo de ajuste de tensão ganancioso guiado por perfil (ou \textit{profile-guided}) que se baseia nos \textit{hot paths} para definir o melhor perfil de consumo de energia para uma dada aplicação de tempo real.} \\ \hline \hline

\multicolumn{1}{|r|}{\textbf{Método(s) utilizados}} & DVFS Intra-Task; Control Flow Graph (CFG); \\ \hline
\multicolumn{1}{|r|}{\textbf{Ferramenta(s)}} & {Os autores não mencionam o uso de ferramentas e / ou \textit{benchmarks}.} \\ \hline \hline

\multicolumn{2}{|c|}{\textbf{Impacto (positivo x negativo)}} \\ \hline
\multicolumn{2}{|p{20cm}|}{O artigo apresentou como ponto positivo uma nova metodologia que realiza a analise dos \textit{hot paths} da aplicação e criam perfis de consumo de energia para cada caminho identificado, visando maximizar os ganhos obtidos com o uso da técnica DVFS intra-tarefa, através da identificação de tempos de folga na dentro da aplicação. Como ponto negativo, a metodologia insere muitos pontos de controle dentro da aplicação e não mostra um estudo sobre os impactos ocasionados pelos \textit{overheads} inseridos.} \\ \hline \hline

\multicolumn{2}{|c|}{\textbf{Validação do método}} \\ \hline
\multicolumn{2}{|p{20cm}|}{A validação da metodologia ocorreu através de provas matemáticas e comparações de desempenhos com outros trabalhos presentes na literatura.} \\ \hline \hline

\multicolumn{2}{|c|}{\textbf{Limitações do método}} \\ \hline
\multicolumn{2}{|p{20cm}|}{A metodologia não mostra estudos sobre os impactos dos \textit{overheads} inseridos estaticamente dentro da aplicação.} \\ \hline \hline

\multicolumn{2}{|c|}{\textbf{Integração de métodos}} \\ \hline
\multicolumn{2}{|p{20cm}|}{Não se aplica} \\ \hline \hline

\multicolumn{2}{|c|}{\textbf{Modo de aplicação do método}} \\ \hline
\multicolumn{2}{|p{20cm}|}{Offline} \\ \hline \hline

\multicolumn{2}{|c|}{\textbf{Perspectivas futuras}} \\ \hline
\multicolumn{2}{|p{20cm}|}{Não identificada} \\ \hline \hline

\multicolumn{2}{|c|}{\textbf{Comentários}} \\ \hline
\multicolumn{2}{|p{20cm}|}{A metodologia proposta não mostra evidências, no artigo, de que fornece suporte para recursos compartilhados e / ou preempções.} \\ \hline
\end{tabular}
}
\end{table}


%**********************************************************
% PUBLICACAO - ID_EXCEL: 195
%**********************************************************
\newpage
\begin{table}[htp] % h:here; t:top; b:bottom; p:page; default:ht
\centering
\caption{Dados extraído da publicação de \cite{Mohan_Mueller_Root_2005_a}.}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{|p{3.8cm}|p{16cm}|}
\hline
\multicolumn{1}{|r|}{\textbf{ID}} & Mohan\_Mueller\_Root\_2005\_a \\ \hline
\multicolumn{1}{|r|}{\textbf{Título}} & ParaScale: Exploiting parametric timing analysis for real-time schedulers and dynamic voltage scaling \\ \hline
\multicolumn{1}{|r|}{\textbf{Autores}} & Mohan S., Mueller F., Hawkins W., Root M., Healy C., Whalley D. \\ \hline
\multicolumn{1}{|r|}{\textbf{Palavras-chave}} & Dynamic voltage scaling; Hard real-time systems; Lower-power consumption; Parametric -analysis; Parametric approach; Real-time schedulers; Static timing analysis; Worst-case execution time; Real time systems; Scheduling; Voltage stabilizing circuits \\ \hline
\multicolumn{1}{|r|}{\textbf{Fonte da publicação}} & Proceedings - Real-Time Systems Symposium \\ \hline
\multicolumn{1}{|r|}{\textbf{Editora}} & IEEE \\ \hline
\multicolumn{1}{|r|}{\textbf{Ano da publicação}} & 2005 \\ \hline \hline

\multicolumn{2}{|c|}{\textbf{Resumo da publicação}} \\ \hline
\multicolumn{2}{|p{20cm}|}{Os autores propõem uma nova técnica chamada \textit{ParaScale}, que permite fazer análises de tempo paramétrico em conjunto com o escalonamento. Essas análises permitem detectar dinamicamente os limites dos \textit{loops} e o limite inferior do WCET (em inglês, \textit{Wrost Case Execution Time}), em tempo real, durante o tempo de execução restante da tarefa. Portanto, o ganho desta metodologia está, principalmente, sobre os tempos de folga obtidos sobre as estruturas de repetição. Dentre os trabalhos catalogados nessa revisão sistemática este foi o primeiro a trabalhar com limites paramétricos de \textit{loops}, permitindo ter um melhor controle dos tempos de folga dentro de estruturas de repetição.} \\ \hline \hline

\multicolumn{1}{|r|}{\textbf{Método(s) utilizados}} & DVFS Intra-Task; \\ \hline
\multicolumn{1}{|r|}{\textbf{Ferramenta(s)}} & {Os autores utilizaram a ferramenta SimpleScalar [Disponível em: \href{http://www.simplescalar.com/}{http://www.simplescalar.com/}]. \newline

Os autores utilizaram os \textit{benchmarks}: \newline
- Adpcm (\textit{Adaptive Differential Pulse Code Modulation}) \newline
- Cnt (\textit{Sum and count of positive and negative numbers in an array}) \newline
- Lms (\textit{An LMS adaptive signal enhancement}) \newline
- Mm (\textit{Matrix Multiplication})} \\ \hline \hline

\multicolumn{2}{|c|}{\textbf{Impacto (positivo x negativo)}} \\ \hline
\multicolumn{2}{|p{20cm}|}{O artigo apresentou como ponto positivo uma nova metodologia para realizar a detecção dinâmica dos limites inferiores dos \textit{loops} e do WCET em tempo de execução. Como ponto negativo, a metodologia não mostra um estudo detalhado sobre os \textit{overheads} inseridos estaticamente nas tarefas.} \\ \hline \hline

\multicolumn{2}{|c|}{\textbf{Validação do método}} \\ \hline
\multicolumn{2}{|p{20cm}|}{A validação da metodologia ocorreu através do uso de ferramentas e \textit{benchmarks} relatados na literatura. Além disso, compara os resultados experimentais com outros trabalhos de referência na área de baixo consumo de energia.} \\ \hline \hline

\multicolumn{2}{|c|}{\textbf{Limitações do método}} \\ \hline
\multicolumn{2}{|p{20cm}|}{A metodologia proposta não mostra um estudo detalhado sobre os \textit{overheads} inseridos estaticamente nas tarefas.} \\ \hline \hline

\multicolumn{2}{|c|}{\textbf{Integração de métodos}} \\ \hline
\multicolumn{2}{|p{20cm}|}{Não se aplica} \\ \hline \hline

\multicolumn{2}{|c|}{\textbf{Modo de aplicação do método}} \\ \hline
\multicolumn{2}{|p{20cm}|}{Híbrida} \\ \hline \hline

\multicolumn{2}{|c|}{\textbf{Perspectivas futuras}} \\ \hline
\multicolumn{2}{|p{20cm}|}{Integrar ao método um mecanismo de detecção automática dos limites superiores dos loops, pois esses limites são definidos estaticamente no código fonte da aplicação.} \\ \hline \hline

\multicolumn{2}{|c|}{\textbf{Comentários}} \\ \hline
\multicolumn{2}{|p{20cm}|}{A metodologia proposta não mostra evidências, no artigo, de que fornece suporte para recursos compartilhados e / ou preempções.} \\ \hline
\end{tabular}
}
\end{table}


%**********************************************************
% PUBLICACAO - ID_EXCEL: 194
%**********************************************************
\newpage
\begin{table}[htp] % h:here; t:top; b:bottom; p:page; default:ht
\centering
\caption{Dados extraído da publicação de \cite{Yi_Yang_2005_a}.}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{|p{3.8cm}|p{16cm}|}
\hline
\multicolumn{1}{|r|}{\textbf{ID}} & Yi\_Yang\_2005\_a \\ \hline
\multicolumn{1}{|r|}{\textbf{Título}} & Optimizing the configuration of dynamic voltage scaling points in real-time applications \\ \hline
\multicolumn{1}{|r|}{\textbf{Autores}} & Yi H., Yang X. \\ \hline
\multicolumn{1}{|r|}{\textbf{Palavras-chave}} & Computer simulation; Electric potential; Energy conservation; Energy efficiency; Energy utilization; Real time systems; Dynamic voltage scaling (DVS); Energy models; Real-time applications; Supply voltage; Program compilers \\ \hline
\multicolumn{1}{|r|}{\textbf{Fonte da publicação}} & 15th International Workshop, PATMOS 2005 \\ \hline
\multicolumn{1}{|r|}{\textbf{Editora}} & Springer \\ \hline
\multicolumn{1}{|r|}{\textbf{Ano da publicação}} & 2005 \\ \hline \hline

\multicolumn{2}{|c|}{\textbf{Resumo da publicação}} \\ \hline
\multicolumn{2}{|p{20cm}|}{Os autores propõem uma metodologia de configuração baseado em um método que constrói o padrão de execução de uma determinada aplicação, também chamado de \textit{Profile-Based Method} já relatado na publicação de \cite{Yi_Yang_Chen_2005_a}. O diferencial desta nova abordagem está em diminuir os \textit{overheads} inseridos pelo compilador no código fonte das aplicações. Esse processo é feito da seguinte forma: primeiro o compilador insere os pontos de escalonamento sem levar em consideração os \textit{overheads}; em seguida, todos os pontos de escalonamento são listados, já levando em consideração os \textit{overheads}; e por fim, os pontos que possuem maiores \textit{overheads} e / ou não trazem redução do consumo de energia para aplicação são excluídos.} \\ \hline \hline

\multicolumn{1}{|r|}{\textbf{Método(s) utilizados}} & DVFS Intra-Task; \\ \hline
\multicolumn{1}{|r|}{\textbf{Ferramenta(s)}} & {Os autores não especificaram o uso de ferramentas e / ou \textit{benchmarks}.} \\ \hline \hline

\multicolumn{2}{|c|}{\textbf{Impacto (positivo x negativo)}} \\ \hline
\multicolumn{2}{|p{20cm}|}{O artigo apresentou como ponto positivo uma nova metodologia para realizar a análise e aplicação de pontos de escalonamento de tensão (VSPs) em aplicações de tempo real. Como ponto negativo, a metodologia não deixa claro se dá suporte a alguns tipos de estruturas como \textit{loops} ocultos e recursões.} \\ \hline \hline

\multicolumn{2}{|c|}{\textbf{Validação do método}} \\ \hline
\multicolumn{2}{|p{20cm}|}{A validação da metodologia ocorreu através de casos de teste criados pelos próprios autores.} \\ \hline \hline

\multicolumn{2}{|c|}{\textbf{Limitações do método}} \\ \hline
\multicolumn{2}{|p{20cm}|}{A metodologia proposta não deixa claro quais são os tipos de estruturas suportadas.} \\ \hline \hline

\multicolumn{2}{|c|}{\textbf{Integração de métodos}} \\ \hline
\multicolumn{2}{|p{20cm}|}{Não se aplica} \\ \hline \hline

\multicolumn{2}{|c|}{\textbf{Modo de aplicação do método}} \\ \hline
\multicolumn{2}{|p{20cm}|}{Offline} \\ \hline \hline

\multicolumn{2}{|c|}{\textbf{Perspectivas futuras}} \\ \hline
\multicolumn{2}{|p{20cm}|}{Fornecer suporte a \textit{loops} ocultos e recursões.} \\ \hline \hline

\multicolumn{2}{|c|}{\textbf{Comentários}} \\ \hline
\multicolumn{2}{|p{20cm}|}{A metodologia proposta não mostra evidências, no artigo, de que fornece suporte para recursos compartilhados e / ou preempções.} \\ \hline
\end{tabular}
}
\end{table}


%**********************************************************
% PUBLICACAO - ID_EXCEL: 193
%**********************************************************
\newpage
\begin{table}[htp] % h:here; t:top; b:bottom; p:page; default:ht
\centering
\caption{Dados extraído da publicação de \cite{Shin_Kim_2005_b}.}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{|p{3.8cm}|p{16cm}|}
\hline
\multicolumn{1}{|r|}{\textbf{ID}} & Shin\_Kim\_2005\_b \\ \hline
\multicolumn{1}{|r|}{\textbf{Título}} & Optimizing intra-task voltage scheduling using data flow analysis \\ \hline
\multicolumn{1}{|r|}{\textbf{Autores}} & Shin D., Kim J. \\ \hline
\multicolumn{1}{|r|}{\textbf{Palavras-chave}} & Control flows; Data flow; Data-flow information; Low power application; Optimization techniques; Slack time; Supply voltages; Voltage scheduling; Voltage-scaling; Algorithms; Computer aided design; Data flow analysis; Data transfer; Energy efficiency; Energy utilization; Motion Picture Experts Group standards; Scheduling; Optimization \\ \hline
\multicolumn{1}{|r|}{\textbf{Fonte da publicação}} & Proceedings of the Asia and South Pacific Design Automation Conference, ASP-DAC \\ \hline
\multicolumn{1}{|r|}{\textbf{Editora}} & IEEE \\ \hline
\multicolumn{1}{|r|}{\textbf{Ano da publicação}} & 2005 \\ \hline \hline

\multicolumn{2}{|c|}{\textbf{Resumo da publicação}} \\ \hline
\multicolumn{2}{|p{20cm}|}{Os autores propõem uma otimização na técnica intraDVS usando informações de fluxo de dados da aplicação de tempo real. A metodologia visa melhorar a eficiência energética antecipando os pontos de escalonamento de tensão (em inglês, \textit{Voltage Scaling Points} - VSPs), baseadas nos resultados de análises do fluxo de dados da aplicação. Essa técnica foi chamada de \textit{LaIntraDVS} (em inglês, Look Ahead IntraDVS). Em outras palavras, o método proposto antecipa os pontos de controle para maximizar os ganhos de energia da técnica intraDVS, como por exemplo: analisar uma estrutura de repetição e predizer quantas interações serão necessárias e aplicar as tensões e frequências ideais para essa bloco de código antes que ele seja realmente executado.} \\ \hline \hline

\multicolumn{1}{|r|}{\textbf{Método(s) utilizados}} & DVFS Intra-Task; \\ \hline
\multicolumn{1}{|r|}{\textbf{Ferramenta(s)}} & {Os autores não especificam a ferramenta utilizada nos experimentos. \newline

Os autores utilizaram os seguintes \textit{benchmarks}: \newline
- MPEG-4 \textit{video encoder} \newline
- MPEG-4 \textit{video decoder}} \\ \hline \hline

\multicolumn{2}{|c|}{\textbf{Impacto (positivo x negativo)}} \\ \hline
\multicolumn{2}{|p{20cm}|}{O artigo apresentou como ponto positivo uma nova metodologia para antecipar (ou predizer) os pontos de escalonamento de tensão (VSPs) visando maximizar os ganhos da técnica intraDVS. Como ponto negativo, a metodologia fornece ganhos mais efetivos apenas quando as distâncias entre os pontos de escalonamento de tensão são grandes.} \\ \hline \hline

\multicolumn{2}{|c|}{\textbf{Validação do método}} \\ \hline
\multicolumn{2}{|p{20cm}|}{A validação da metodologia ocorreu através do uso de ferramentas e \textit{benchmarks} relatados na literatura. Além disso, compara os resultados experimentais com outros trabalhos de referência na área de baixo consumo de energia.} \\ \hline \hline

\multicolumn{2}{|c|}{\textbf{Limitações do método}} \\ \hline
\multicolumn{2}{|p{20cm}|}{A metodologia fornece ganhos mais efetivos apenas quando as distâncias entre os pontos de escalonamento de tensão são grandes.} \\ \hline \hline

\multicolumn{2}{|c|}{\textbf{Integração de métodos}} \\ \hline
\multicolumn{2}{|p{20cm}|}{Não se aplica} \\ \hline \hline

\multicolumn{2}{|c|}{\textbf{Modo de aplicação do método}} \\ \hline
\multicolumn{2}{|p{20cm}|}{Offline} \\ \hline \hline

\multicolumn{2}{|c|}{\textbf{Perspectivas futuras}} \\ \hline
\multicolumn{2}{|p{20cm}|}{Fornecer suporte a outros tipos de estruturas, como: \textit{loops} ocultos e recursões.} \\ \hline \hline

\multicolumn{2}{|c|}{\textbf{Comentários}} \\ \hline
\multicolumn{2}{|p{20cm}|}{
- Este é um dos primeiros trabalhos a antecipar (ou predizer) pontos de escalonamento de tensão (VSPs).

- A metodologia proposta não mostra evidências, no artigo, de que fornece suporte para recursos compartilhados e / ou preempções.} \\ \hline
\end{tabular}
}
\end{table}


%**********************************************************
% PUBLICACAO - ID_EXCEL: 192
%**********************************************************
\newpage
\begin{table}[htp] % h:here; t:top; b:bottom; p:page; default:ht
\centering
\caption{Dados extraído da publicação de \cite{Seo_Kim_Dutt_2005_a}.}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{|p{3.8cm}|p{16cm}|}
\hline
\multicolumn{1}{|r|}{\textbf{ID}} & Seo\_Kim\_Dutt\_2005\_a \\ \hline
\multicolumn{1}{|r|}{\textbf{Título}} & Optimal integration of inter-task and intra-task dynamic voltage scaling techniques for hard real-time applications \\ \hline
\multicolumn{1}{|r|}{\textbf{Autores}} & Seo J., Kim T., Dutt N.D. \\ \hline
\multicolumn{1}{|r|}{\textbf{Palavras-chave}} & Dynamic voltage scaling (DVS); Energy minimization; Polynomial time; Computation theory; Energy efficiency; Energy utilization; Optimal systems; Optimization; Polynomial approximation; Problem solving; Real time systems; Voltage control \\ \hline
\multicolumn{1}{|r|}{\textbf{Fonte da publicação}} & IEEE/ACM International Conference on Computer-Aided Design, Digest of Technical Papers, ICCAD \\ \hline
\multicolumn{1}{|r|}{\textbf{Editora}} & IEEE \\ \hline
\multicolumn{1}{|r|}{\textbf{Ano da publicação}} & 2005 \\ \hline \hline

\multicolumn{2}{|c|}{\textbf{Resumo da publicação}} \\ \hline
\multicolumn{2}{|p{20cm}|}{Os autores propõe uma nova técnica DVS que combinam as técnicas DVS intra-tarefa e inter-tarefa, chamada de \textit{DVS-intgr}. Essa metodologia examina os limites inferiores de consumo de energia baseado na técnica DVS intra-tarefa (parte dessa metodologia foi inspirada no trabalho de \cite{Shin_Kim_Lee_2001_a}) e com essas propriedades foram definidos os tempos de execução ideais de cada tarefa. Em seguida, as tarefas são divididas em vários grupos de trabalho de tal forma que cada tarefa possa ser executada dentro do limite preestabelecido para cada grupo, através da utilização da técnica DVS inter-tarefa melhorada para produzir o melhor escalonamento entre elas de forma que haja a redução no consumo de energia e garantindo que nenhum premissa temporal seja violada.} \\ \hline \hline

\multicolumn{1}{|r|}{\textbf{Método(s) utilizados}} & DVFS Intra-Task; DVFS Inter-Task; \\ \hline
\multicolumn{1}{|r|}{\textbf{Ferramenta(s)}} & {O autor utilizou a ferramenta TGFF v3.0.} \\ \hline \hline

\multicolumn{2}{|c|}{\textbf{Impacto (positivo x negativo)}} \\ \hline
\multicolumn{2}{|p{20cm}|}{O artigo apresentou como ponto positivo uma nova metodologia que realizou a integração das técnicas DVS intra-tarefa com a inter-tarefa e introduziu o conceito de grupo de tarefas para maximizar os resultados obtidos com o uso da técnica DVFS. Como ponto negativo, a metodologia não apresenta um estudo detalhado sobre os overheads inseridos na aplicação.} \\ \hline \hline

\multicolumn{2}{|c|}{\textbf{Validação do método}} \\ \hline
\multicolumn{2}{|p{20cm}|}{A validação da metodologia ocorreu através do uso de ferramenta relatada na literatura. Além disso, compara os resultados experimentais com outros trabalhos de referência na área de baixo consumo de energia.} \\ \hline \hline

\multicolumn{2}{|c|}{\textbf{Limitações do método}} \\ \hline
\multicolumn{2}{|p{20cm}|}{A metodologia não mostra os impactos dos overheads inseridos na aplicação (tanto intra-tarefa quanto inter-tarefa).} \\ \hline \hline

\multicolumn{2}{|c|}{\textbf{Integração de métodos}} \\ \hline
\multicolumn{2}{|p{20cm}|}{Integrou as técnica DVFS intra-tarefa com a técnica DVFS inter-tarefa} \\ \hline \hline

\multicolumn{2}{|c|}{\textbf{Modo de aplicação do método}} \\ \hline
\multicolumn{2}{|p{20cm}|}{Híbrida} \\ \hline \hline

\multicolumn{2}{|c|}{\textbf{Perspectivas futuras}} \\ \hline
\multicolumn{2}{|p{20cm}|}{Mostrar um estudo mais detalhado sobre os overheads introduzidos pela metodologia.} \\ \hline \hline

\multicolumn{2}{|c|}{\textbf{Comentários}} \\ \hline
\multicolumn{2}{|p{20cm}|}{A metodologia proposta não mostra evidências, no artigo, de que fornece suporte para recursos compartilhados e / ou preempções.} \\ \hline
\end{tabular}
}
\end{table}


%**********************************************************
% PUBLICACAO - ID_EXCEL: 191
%**********************************************************
\newpage
\begin{table}[htp] % h:here; t:top; b:bottom; p:page; default:ht
\centering
\caption{Dados extraído da publicação de \cite{Cassandras_Zhuang_2005_a}.}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{|p{3.8cm}|p{16cm}|}
\hline
\multicolumn{1}{|r|}{\textbf{ID}} & Cassandras\_Zhuang\_2005\_a \\ \hline
\multicolumn{1}{|r|}{\textbf{Título}} & Optimal dynamic voltage scaling for wireless sensor nodes with real-time constraints \\ \hline
\multicolumn{1}{|r|}{\textbf{Autores}} & Cassandras C.G., Zhuang S. \\ \hline
\multicolumn{1}{|r|}{\textbf{Palavras-chave}} & Product monitoring; Scalability; Voltage scaling; Computer simulation; Control equipment; Inventory control; Nonlinear programming; Real time systems; Sensors; Voltage control \\ \hline
\multicolumn{1}{|r|}{\textbf{Fonte da publicação}} & Proc. SPIE 5999, Intelligent Systems in Design and Manufacturing VI \\ \hline
\multicolumn{1}{|r|}{\textbf{Editora}} & SPIE - Digital Library \\ \hline
\multicolumn{1}{|r|}{\textbf{Ano da publicação}} & 2005 \\ \hline \hline

\multicolumn{2}{|c|}{\textbf{Resumo da publicação}} \\ \hline
\multicolumn{2}{|p{20cm}|}{Os autores propõe um controle intra-tarefa para minimizar o consumo de energia dentro do contexto de rede de sensores sem fio, processando tarefas de tempo real críticas. As variáveis de controle são basicamente os tempos de processamento das tarefas de tempo real, onde cada um desses tempos estão associados a diferentes níveis de tensão. O controle intra-tarefa é baseado na exploração das propriedades dos caminhos de execução ideais. Além disso os autores mostram em seus experimentos que soluções intra-tarefa minimizam mais energia que as soluções inter-tarefa.} \\ \hline \hline

\multicolumn{1}{|r|}{\textbf{Método(s) utilizados}} & DVFS Intra-Task; \\ \hline
\multicolumn{1}{|r|}{\textbf{Ferramenta(s)}} & {O autor não mencionou o uso de nenhuma ferramenta e nenhum \textit{benchmark}.} \\ \hline \hline

\multicolumn{2}{|c|}{\textbf{Impacto (positivo x negativo)}} \\ \hline
\multicolumn{2}{|p{20cm}|}{O artigo apresentou como ponto positivo uma nova metodologia baseada na técnica DVFS intra-tarefa aplicada no contexto de redes de sensores sem fio, processando tarefas com restrições temporais. Como ponto negativo, a metodologia não mostra estudos sobre os impactos dos overheads inseridos nas tarefas.} \\ \hline \hline

\multicolumn{2}{|c|}{\textbf{Validação do método}} \\ \hline
\multicolumn{2}{|p{20cm}|}{A validação da metodologia ocorreu através de casos de teste criados pelo próprio autor. Além disso, compara os resultados experimentais com outros trabalhos de referência na área de baixo consumo de energia.} \\ \hline \hline

\multicolumn{2}{|c|}{\textbf{Limitações do método}} \\ \hline
\multicolumn{2}{|p{20cm}|}{A metodologia não mostra um estudo sobre os overheads inseridos estaticamente dentro das tarefas.} \\ \hline \hline

\multicolumn{2}{|c|}{\textbf{Integração de métodos}} \\ \hline
\multicolumn{2}{|p{20cm}|}{Não se aplica} \\ \hline \hline

\multicolumn{2}{|c|}{\textbf{Modo de aplicação do método}} \\ \hline
\multicolumn{2}{|p{20cm}|}{Híbrida} \\ \hline \hline

\multicolumn{2}{|c|}{\textbf{Perspectivas futuras}} \\ \hline
\multicolumn{2}{|p{20cm}|}{Mostrar um estudo mais detalhado sobre os overheads introduzidos pelo metodologia.} \\ \hline \hline

\multicolumn{2}{|c|}{\textbf{Comentários}} \\ \hline
\multicolumn{2}{|p{20cm}|}{A metodologia proposta não mostra evidências, no artigo, de que fornece suporte para recursos compartilhados e / ou preempções.} \\ \hline
\end{tabular}
}
\end{table}


%**********************************************************
% PUBLICACAO - ID_EXCEL: 185
%**********************************************************
\newpage
\begin{table}[htp] % h:here; t:top; b:bottom; p:page; default:ht
\centering
\caption{Dados extraído da publicação de \cite{Kumar_Manimaran_2005_a}.}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{|p{3.8cm}|p{16cm}|}
\hline
\multicolumn{1}{|r|}{\textbf{ID}} & Kumar\_Manimaran\_2005\_a \\ \hline
\multicolumn{1}{|r|}{\textbf{Título}} & An intra-task DVS algorithm exploiting program path locality for real-time embedded systems \\ \hline
\multicolumn{1}{|r|}{\textbf{Autores}} & Kumar G.S.A., Manimaran G. \\ \hline
\multicolumn{1}{|r|}{\textbf{Palavras-chave}} & Computer simulation; Embedded systems; Energy utilization; Real time systems; Scheduling; Dynamic Voltage Scheduling (DVS); Frequently executed paths; Real-time embedded systems; Algorithms \\ \hline
\multicolumn{1}{|r|}{\textbf{Fonte da publicação}} & 12th International Conference on High Performance Computing, HiPC 2005; \\ \hline
\multicolumn{1}{|r|}{\textbf{Editora}} & Springer \\ \hline
\multicolumn{1}{|r|}{\textbf{Ano da publicação}} & 2005 \\ \hline \hline

\multicolumn{2}{|c|}{\textbf{Resumo da publicação}} \\ \hline
\multicolumn{2}{|p{20cm}|}{Os autores propõem um novo algoritmo DVS intra-tarefa de consumo de energia consciente cujo o objetivo central é explorar os caminhos mais comuns e frequentemente executados dentro de uma aplicação de tempo real. Esse algoritmo foi chamado de CHP (em inglês, \textit{Common Hot Path}). Essa metodologia considera todos os caminhos mais executados (ou \textit{hot-paths}), principio também utilizado nos trabalhos de \cite{Shin_Kim_2001_a}, \cite{Seo_Kim_Chung_2004_a}, \cite{Yi_Yang_Chen_2005_a} e \cite{Shin_Kim_2005_a}, e para cada um deles são atribuídas probabilidades que irão indicar os caminhos mais utilizados. Dessa forma, a metodologia consegue combinar todos os \textit{hot paths} em um único caminho base que é comum em comprimento com a maioria dos \textit{hot paths}, assim é possível descobrir qual o caminho que leva a melhores taxas de minimização do consumo de energia, pois nem sempre o caminho mais curto é o mais eficaz para minimização do consumo de energia.} \\ \hline \hline

\multicolumn{1}{|r|}{\textbf{Método(s) utilizados}} & DVFS Intra-Task; Control Flow Graph (CFG); \\ \hline
\multicolumn{1}{|r|}{\textbf{Ferramenta(s)}} & {Os autores não mencionam o uso de nenhuma ferramenta. \newline

Os autores utilizam o seguinte \textit{benchmark}: \newline
- MPEG-4 \textit{video decoder \& encoder}} \\ \hline \hline

\multicolumn{2}{|c|}{\textbf{Impacto (positivo x negativo)}} \\ \hline
\multicolumn{2}{|p{20cm}|}{O artigo apresentou como ponto positivo uma nova metodologia que obtém os caminhos de execução com menores consumo de energia, através do uso de probabilidade e caminhos mais executados. Como ponto negativo, a metodologia tem dificuldades para lhe dar com alguns tipos de estruturas, como \textit{loops} sem profundidade.} \\ \hline \hline

\multicolumn{2}{|c|}{\textbf{Validação do método}} \\ \hline
\multicolumn{2}{|p{20cm}|}{A validação da metodologia ocorreu através do uso de \textit{benchmarks} relatados na literatura. Além disso, compara os resultados experimentais com outros trabalhos de referência na área de baixo consumo de energia.} \\ \hline \hline

\multicolumn{2}{|c|}{\textbf{Limitações do método}} \\ \hline
\multicolumn{2}{|p{20cm}|}{A metodologia tem dificuldades para lhe dar com alguns tipos de estruturas, como por exemplo: \textit{loops} sem profundidade.} \\ \hline \hline

\multicolumn{2}{|c|}{\textbf{Integração de métodos}} \\ \hline
\multicolumn{2}{|p{20cm}|}{Não se aplica} \\ \hline \hline

\multicolumn{2}{|c|}{\textbf{Modo de aplicação do método}} \\ \hline
\multicolumn{2}{|p{20cm}|}{Offline} \\ \hline \hline

\multicolumn{2}{|c|}{\textbf{Perspectivas futuras}} \\ \hline
\multicolumn{2}{|p{20cm}|}{O autor pretende mostrar que utilizando informações offline, como por exemplo a quantidade de interações de um \textit{loop}, é possível minimizar o consumo de energia.} \\ \hline \hline

\multicolumn{2}{|c|}{\textbf{Comentários}} \\ \hline
\multicolumn{2}{|p{20cm}|}{A metodologia proposta não mostra evidências, no artigo, de que fornece suporte para recursos compartilhados e / ou preempções.} \\ \hline
\end{tabular}
}
\end{table}


%**********************************************************
% PUBLICACAO - ID_EXCEL: 181
%**********************************************************
\newpage
\begin{table}[htp] % h:here; t:top; b:bottom; p:page; default:ht
\centering
\caption{Dados extraído da publicação de \cite{Gheorghita_2005_a}.}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{|p{3.8cm}|p{16cm}|}
\hline
\multicolumn{1}{|r|}{\textbf{ID}} & Gheorghita\_2005\_a \\ \hline
\multicolumn{1}{|r|}{\textbf{Título}} & Intra-task scenario-aware voltage scheduling \\ \hline
\multicolumn{1}{|r|}{\textbf{Autores}} & Gheorghita S.V., Basten T., Corporaal H. \\ \hline
\multicolumn{1}{|r|}{\textbf{Palavras-chave}} & Dynamic Voltage Scheduling; Real-Time; Scenarios; WCET \\ \hline
\multicolumn{1}{|r|}{\textbf{Fonte da publicação}} & CASES 2005: International Conference on Compilers, Architecture, and Synthesis for Embedded Systems \\ \hline
\multicolumn{1}{|r|}{\textbf{Editora}} & ACM \\ \hline
\multicolumn{1}{|r|}{\textbf{Ano da publicação}} & 2005 \\ \hline \hline

\multicolumn{2}{|c|}{\textbf{Resumo da publicação}} \\ \hline
\multicolumn{2}{|p{20cm}|}{Os autores propõem uma abordagem proativa que visa melhorar a performance do algoritmo de escalonamento intra-tarefa, explorando os tempos de folga que aparecem em tempo de execução, em seguida repassa para o processador através trechos de código inseridos na aplicação original, chamados de pontos de escalonamento de tensão ou VSPs (em inglês, \textit{Voltage Scaling Points}). Essa abordagem consiste, basicamente, em quatro etapas: (1) identificar os parâmetros que poderiam ter um impacto sobre o tempo de execução da aplicação; (2) calcular o máximo de impacto destes parâmetros sobre o WCEC da aplicação; (3) particionar o aplicativo em possíveis cenários, considerando-se esses parâmetros, juntamente com o seu impacto, e selecionando apenas cenários que, isoladamente, reduzir o consumo de energia; por fim, (4) computar o escalonamento DVS para cada cenário selecionado no estágio 3 e combiná-los com o escalonamento global da aplicação de tempo real.} \\ \hline \hline

\multicolumn{1}{|r|}{\textbf{Método(s) utilizados}} & DVFS Intra-Task; Control Flow Graph (CFG); \\ \hline
\multicolumn{1}{|r|}{\textbf{Ferramenta(s)}} & {Os autores não mencionaram o uso de nenhuma ferramenta. \newline

Os autores utilizaram os seguintes \textit{benchmarks}: \newline
- MP3 \textit{decoder} \newline
- H.263 \textit{decoder}} \\ \hline \hline

\multicolumn{2}{|c|}{\textbf{Impacto (positivo x negativo)}} \\ \hline
\multicolumn{2}{|p{20cm}|}{O artigo apresentou como ponto positivo uma nova metodologia de análise de CFGs para explorar os tempos de folga da tarefa. Como ponto negativo, a metodologia tem dificuldades para lhe dar com alguns tipos de estruturas (exemplo: \textit{loops} sem profundidade, \textit{loops} ocultos e recursões).} \\ \hline \hline

\multicolumn{2}{|c|}{\textbf{Validação do método}} \\ \hline
\multicolumn{2}{|p{20cm}|}{A validação da metodologia ocorreu através do uso de \textit{benchmarks} relatados na literatura.} \\ \hline \hline

\multicolumn{2}{|c|}{\textbf{Limitações do método}} \\ \hline
\multicolumn{2}{|p{20cm}|}{A metodologia não prever todos os tipos de estruturas de dados (como \textit{loops} sem profundidade, \textit{loops} ocultos e recursões).} \\ \hline \hline

\multicolumn{2}{|c|}{\textbf{Integração de métodos}} \\ \hline
\multicolumn{2}{|p{20cm}|}{Não se aplica} \\ \hline \hline

\multicolumn{2}{|c|}{\textbf{Modo de aplicação do método}} \\ \hline
\multicolumn{2}{|p{20cm}|}{Híbrido} \\ \hline \hline

\multicolumn{2}{|c|}{\textbf{Perspectivas futuras}} \\ \hline
\multicolumn{2}{|p{20cm}|}{O autor pretende introduzir uma abordagem probabilística para tentar prever qual bloco da aplicação serão executados e introduzir a técnica DVFS inter-tarefas para maximizar os ganhos da metodologia proposta neste trabalho.} \\ \hline \hline

\multicolumn{2}{|c|}{\textbf{Comentários}} \\ \hline
\multicolumn{2}{|p{20cm}|}{
- O autor insere o conceito de abordagem proativa, ou seja, ela consegue prever para um determinado bloco de código quais serão as tensões e frequências ideais a serem utilizadas (exemplo: se um \textit{loop} tem no máximo 50 interações e só executará 20 interações, então será possível ajustar as tensões e frequências do processador antes de entrar no \textit{loop}).

- A metodologia proposta não mostra evidências, no artigo, de que fornece suporte para recursos compartilhados e / ou preempções.} \\ \hline
\end{tabular}
}
\end{table}


%**********************************************************
% PUBLICACAO - ID_EXCEL: 171
%**********************************************************
\newpage
\begin{table}[htp] % h:here; t:top; b:bottom; p:page; default:ht
\centering
\caption{Dados extraído da publicação de \cite{Yi_Yang_2006_a}.}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{|p{3.8cm}|p{16cm}|}
\hline
\multicolumn{1}{|r|}{\textbf{ID}} & Yi\_Yang\_2006\_a \\ \hline
\multicolumn{1}{|r|}{\textbf{Título}} & Toward the optimal configuration of dynamic voltage scaling points in real-time applications \\ \hline
\multicolumn{1}{|r|}{\textbf{Autores}} & Yi H.-Z., Yang X.-J. \\ \hline
\multicolumn{1}{|r|}{\textbf{Palavras-chave}} & Energy-aware systems; Languages and compilers; Low-power design \\ \hline
\multicolumn{1}{|r|}{\textbf{Fonte da publicação}} & Journal of Computer Science and Technology \\ \hline
\multicolumn{1}{|r|}{\textbf{Editora}} & Springer \\ \hline
\multicolumn{1}{|r|}{\textbf{Ano da publicação}} & 2006 \\ \hline \hline

\multicolumn{2}{|c|}{\textbf{Resumo da publicação}} \\ \hline
\multicolumn{2}{|p{20cm}|}{Os autores apresentam uma metodologia de configuração ótima de pontos de escalonamento de tensão dinâmicos sem \textit{overheads} de escalonamento de tensão, onde tomaram como base os trabalhos de \cite{Aboughazaleh_2003_b} e \cite{Aboughazaleh_2003_a}. Com essa metodologia os autores conseguiram introduzir a menor quantidade necessária de pontos de escalonamento de tensão para melhor aproveitar os tempos de folga da aplicação e, além disso, provaram teoricamente todos os modelos e teoremas matemáticos definidos na metodologia, sempre visando a otimização ideal de energia.} \\ \hline \hline

\multicolumn{1}{|r|}{\textbf{Método(s) utilizados}} & DVFS Intra-Task; \\ \hline
\multicolumn{1}{|r|}{\textbf{Ferramenta(s)}} & {Os autores não especificaram a ferramenta utilizada e nem faz referência ao uso de algum \textit{benchmark}.} \\ \hline \hline

\multicolumn{2}{|c|}{\textbf{Impacto (positivo x negativo)}} \\ \hline
\multicolumn{2}{|p{20cm}|}{O artigo apresentou como ponto positivo uma nova heurística de inserção de pontos de escalonamento de tensão dentro de aplicações de tempo real. Como ponto negativo, a metodologia não deixa claro os tipos de estruturas suportadas pelo compilador responsável por inserir os pontos de controle no código fonte da tarefa.} \\ \hline \hline

\multicolumn{2}{|c|}{\textbf{Validação do método}} \\ \hline
\multicolumn{2}{|p{20cm}|}{A validação da metodologia ocorreu através de provas matemáticas e pelo uso de casos de testes definidos pelo próprio autor.} \\ \hline \hline

\multicolumn{2}{|c|}{\textbf{Limitações do método}} \\ \hline
\multicolumn{2}{|p{20cm}|}{A metodologia não prever todos os tipos de estruturas de dados (como as recursões) e não leva em consideração preempções.} \\ \hline \hline

\multicolumn{2}{|c|}{\textbf{Integração de métodos}} \\ \hline
\multicolumn{2}{|p{20cm}|}{Não se aplica} \\ \hline \hline

\multicolumn{2}{|c|}{\textbf{Modo de aplicação do método}} \\ \hline
\multicolumn{2}{|p{20cm}|}{Offline} \\ \hline \hline

\multicolumn{2}{|c|}{\textbf{Perspectivas futuras}} \\ \hline
\multicolumn{2}{|p{20cm}|}{O autor propõe realizar estudos mais detalhados quando os \textit{overheads} de escalonamento de tensão forem muito grandes.} \\ \hline \hline

\multicolumn{2}{|c|}{\textbf{Comentários}} \\ \hline
\multicolumn{2}{|p{20cm}|}{A metodologia proposta não mostra evidências, no artigo, de que fornece suporte para recursos compartilhados e / ou preempções.} \\ \hline
\end{tabular}
}
\end{table}


%**********************************************************
% PUBLICACAO - ID_EXCEL: 170
%**********************************************************
\newpage
\begin{table}[htp] % h:here; t:top; b:bottom; p:page; default:ht
\centering
\caption{Dados extraído da publicação de \cite{Xian_Lu_2006_a}.}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{|p{3.8cm}|p{16cm}|}
\hline
\multicolumn{1}{|r|}{\textbf{ID}} & Xian\_Lu\_2006\_a \\ \hline
\multicolumn{1}{|r|}{\textbf{Título}} & Dynamic voltage scaling for multitasking real-time systems with uncertain execution time \\ \hline
\multicolumn{1}{|r|}{\textbf{Autores}} & Xian C., Lu Y.-H. \\ \hline
\multicolumn{1}{|r|}{\textbf{Palavras-chave}} & Dynamic voltage scaling; Hard real-time; Low energy; Multitasking; Probability \\ \hline
\multicolumn{1}{|r|}{\textbf{Fonte da publicação}} & Proceedings of the ACM Great Lakes Symposium on VLSI, GLSVLSI \\ \hline
\multicolumn{1}{|r|}{\textbf{Editora}} & ACM \\ \hline
\multicolumn{1}{|r|}{\textbf{Ano da publicação}} & 2006 \\ \hline \hline

\multicolumn{2}{|c|}{\textbf{Resumo da publicação}} \\ \hline
\multicolumn{2}{|p{20cm}|}{Os autores propõem uma abordagem que visa integrar as técnicas de escalonamento de tensão intra-tarefa e inter-tarefa. O conceito principal do método proposto é que cada tarefa possa contribuir com informações individuais para que seja possível melhorar o escalonamento individual das demais tarefas em execução, sempre tomando como base as informações globais passadas pelas demais tarefas. Dessa forma, a abordagem é dividida, basicamente, em duas etapas: (1) É calculado estatisticamente o escalonamento de frequência ótimo para múltiplas tarefas periódicas utilizando o escalonamento EDF (em inglês, \textit{Earliest Deadline First}) para processadores que conseguem mudar suas frequências de forma contínua; e (2) para processadores que possuem uma faixa limitada de frequências discretas, é apresentado um algoritmo heurístico específico para construção do escalonamento de frequência baseado em informações de distribuição de probabilidade e restrições de escalonabilidade globais.} \\ \hline \hline

\multicolumn{1}{|r|}{\textbf{Método(s) utilizados}} & DVFS Intra-Task; DVFS Inter-Task; \\ \hline
\multicolumn{1}{|r|}{\textbf{Ferramenta(s)}} & {Os autores não utilizaram nenhuma ferramenta específica. \newline

Os autores utilizaram os \textit{benchmarks}: \newline
- MPEG \textit{video decoder} \newline
- MP3 \textit{audio decoder} \newline
- H263 \textit{video decoder} \newline
- GSM \textit{speech encoder}} \\ \hline \hline

\multicolumn{2}{|c|}{\textbf{Impacto (positivo x negativo)}} \\ \hline
\multicolumn{2}{|p{20cm}|}{O artigo apresentou como ponto positivo uma metodologia que integra as técnicas DVFS intra-tarefa com a técnica DVFS inter-tarefa, dando suporte a preempções. Como ponto negativo, a metodologia não prever os \textit{overheads} ocasioandos em tempo de execução.} \\ \hline \hline

\multicolumn{2}{|c|}{\textbf{Validação do método}} \\ \hline
\multicolumn{2}{|p{20cm}|}{A validação da metodologia ocorreu pelo uso de \textit{benchmarks} relatados na literatura. Além disso, compara os resultados experimentais com outros trabalhos de referência na área de baixo consumo de energia.} \\ \hline \hline

\multicolumn{2}{|c|}{\textbf{Limitações do método}} \\ \hline
\multicolumn{2}{|p{20cm}|}{A metodologia não prever os overheads ocasionados em tempo de execução e nem possíveis interferências entre tarefas.} \\ \hline \hline

\multicolumn{2}{|c|}{\textbf{Integração de métodos}} \\ \hline
\multicolumn{2}{|p{20cm}|}{Integrou as técnicas DVFS intra-tarefa com a técnica DVFS inter-tarefa.} \\ \hline \hline

\multicolumn{2}{|c|}{\textbf{Modo de aplicação do método}} \\ \hline
\multicolumn{2}{|p{20cm}|}{Híbrida} \\ \hline \hline

\multicolumn{2}{|c|}{\textbf{Perspectivas futuras}} \\ \hline
\multicolumn{2}{|p{20cm}|}{O autor propõe realizar análises de sensibilidade sobre os tamanhos das tarefas.} \\ \hline \hline

\multicolumn{2}{|c|}{\textbf{Comentários}} \\ \hline
\multicolumn{2}{|p{20cm}|}{A metodologia aborda modelo de tarefas preemptivos, mas não deixa claro como é feito esse suporte. Quanto aos recursos compartilhados, a metodologia proposta não dá suporte.} \\ \hline
\end{tabular}
}
\end{table}


%**********************************************************
% PUBLICACAO - ID_EXCEL: 168
%**********************************************************
\newpage
\begin{table}[htp] % h:here; t:top; b:bottom; p:page; default:ht
\centering
\caption{Dados extraído da publicação de \cite{Hong_Yoo_Choi_Kong_2006_a}.}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{|p{3.8cm}|p{16cm}|}
\hline
\multicolumn{1}{|r|}{\textbf{ID}} & Hong\_Yoo\_Choi\_Kong\_2006\_a \\ \hline
\multicolumn{1}{|r|}{\textbf{Título}} & Runtime distribution-aware dynamic voltage scaling \\ \hline
\multicolumn{1}{|r|}{\textbf{Autores}} & Hong S., Yoo S., Jin H., Choi K.-M., Kong J.-T., Eo S.-K. \\ \hline
\multicolumn{1}{|r|}{\textbf{Palavras-chave}} & Basic blocks; Computer-aided design; Dynamic voltage scaling (DVS); Energy reductions; execution cycles; Experimental results; international conferences; Minimal energy; MPEG-4 decoder; Multimedia software; Performance level (PL); Run time; Software runtime; Worst case execution; Worst case execution cycles; BASIC (programming language); Decoding; Design; Energy policy; Multimedia systems; Voltage stabilizing circuits; Computer software \\ \hline
\multicolumn{1}{|r|}{\textbf{Fonte da publicação}} & IEEE/ACM International Conference on Computer-Aided Design, Digest of Technical Papers, ICCAD \\ \hline
\multicolumn{1}{|r|}{\textbf{Editora}} & IEEE \\ \hline
\multicolumn{1}{|r|}{\textbf{Ano da publicação}} & 2006 \\ \hline \hline

\multicolumn{2}{|c|}{\textbf{Resumo da publicação}} \\ \hline
\multicolumn{2}{|p{20cm}|}{Os autores propõem uma nova técnica de escalonamento de tensão (DVS) intra-tarefa que não visa apenas explorar as distribuições de tempo de execução da aplicação, mas também o fluxo de dados e a arquitetura. Em outras palavras, essa abordagem utiliza os dados da aplicação e da arquitetura para predizer o RWCEC e aplicar com antecedência as tensões e frequências ideais no processador. Portanto, com este trabalho os autores introduziram o conceito de perfil estatístico de ciclos de execução dentro da técnica DVS intra-tarefa ao invés de ciclos de execução no pior caso (WCEC).} \\ \hline \hline

\multicolumn{1}{|r|}{\textbf{Método(s) utilizados}} & DVFS Intra-Task; \\ \hline
\multicolumn{1}{|r|}{\textbf{Ferramenta(s)}} & {O autor utilizou a ferramenta MaxSimTechnology,ARM Co. Ltd [Não disponível para download (\href{http://www.arm.com/products/DevTools/}{http://www.arm.com/products/DevTools/})]. \newline

O autor utilizou os \textit{benchmarks}: \newline
- H.264 Decoder. \newline
- MPEG4 Decoder.} \\ \hline \hline

\multicolumn{2}{|c|}{\textbf{Impacto (positivo x negativo)}} \\ \hline
\multicolumn{2}{|p{20cm}|}{O artigo apresentou como ponto positivo uma metodologia que cria perfis estatísticos com base nos caminhos de execução da tarefa. Como ponto negativo, os autores não deixam claro quais as estruturas de dados sua metodologia suporta.} \\ \hline \hline

\multicolumn{2}{|c|}{\textbf{Validação do método}} \\ \hline
\multicolumn{2}{|p{20cm}|}{A validação da metodologia ocorreu pelo uso de de ferramenta e \textit{benchmarks} descritos na literatura.} \\ \hline \hline

\multicolumn{2}{|c|}{\textbf{Limitações do método}} \\ \hline
\multicolumn{2}{|p{20cm}|}{A metodologia não deixa claro quais tipos de estruturas sua metodologia suporta, como por exemplo: recursos, \textit{loops} ocultos, invariantes de \textit{loops}, etc.} \\ \hline \hline

\multicolumn{2}{|c|}{\textbf{Integração de métodos}} \\ \hline
\multicolumn{2}{|p{20cm}|}{Não se aplica} \\ \hline \hline

\multicolumn{2}{|c|}{\textbf{Modo de aplicação do método}} \\ \hline
\multicolumn{2}{|p{20cm}|}{Offline} \\ \hline \hline

\multicolumn{2}{|c|}{\textbf{Perspectivas futuras}} \\ \hline
\multicolumn{2}{|p{20cm}|}{O autor propõe melhorar a eficiência da metodologia de acordo com o perfil de tempo de execução e explorar as correlações entre blocos de códigos arbitrários.} \\ \hline \hline

\multicolumn{2}{|c|}{\textbf{Comentários}} \\ \hline
\multicolumn{2}{|p{20cm}|}{A metodologia proposta não mostra evidências, no artigo, de que fornece suporte para recursos compartilhados e / ou preempções.} \\ \hline
\end{tabular}
}
\end{table}


%**********************************************************
% PUBLICACAO - ID_EXCEL: 162
%**********************************************************
\newpage
\begin{table}[htp] % h:here; t:top; b:bottom; p:page; default:ht
\centering
\caption{Dados extraído da publicação de \cite{Zhang_2006_a}.}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{|p{3.8cm}|p{16cm}|}
\hline
\multicolumn{1}{|r|}{\textbf{ID}} & Zhang\_2006\_a \\ \hline
\multicolumn{1}{|r|}{\textbf{Título}} & Energy-efficient task scheduling algorithm for mobile terminal \\ \hline
\multicolumn{1}{|r|}{\textbf{Autores}} & Zhang L., Qi D. \\ \hline
\multicolumn{1}{|r|}{\textbf{Palavras-chave}} & Dynamic voltage scaling; Embedded system; Energy minimization; Hybird genetic algorithm; Task sheduling \\ \hline
\multicolumn{1}{|r|}{\textbf{Fonte da publicação}} & IET Conference Publications \\ \hline
\multicolumn{1}{|r|}{\textbf{Editora}} & IET Digital Library \\ \hline
\multicolumn{1}{|r|}{\textbf{Ano da publicação}} & 2006 \\ \hline \hline

\multicolumn{2}{|c|}{\textbf{Resumo da publicação}} \\ \hline
\multicolumn{2}{|p{20cm}|}{Os autores propõem um algoritmo de escalonamento de tarefas baseado em otimizações genéticas para diminuir o consumo de energia quando são especificados os deadlines e os ciclos de execução das tarefas. Esse algoritmo genético híbrido integra as técnicas inter e intra tarefas visando mensurar o pWCEC (em inglês, \textit{Probabilistic Worst-Case Execution Time}), a fim de encontrar o melhor coeficiente de escalonamento das tarefas de forma que todas as restrições temporais sejam obedecidas e ao mesmo tempo se obtenha uma minimização do consumo de energia do processador.} \\ \hline \hline

\multicolumn{1}{|r|}{\textbf{Método(s) utilizados}} & DVFS Intra-Task; DVFS Inter-Task; \\ \hline
\multicolumn{1}{|r|}{\textbf{Ferramenta(s)}} & {Os autores utilizaram a ferramenta: \newline
- Sim-Panalyzer \textit{performance / power simulator} [Ferramenta não disponível para download - Site fora do ar (\href{http://www.eecs.umich.edu/~panalyzer}{http://www.eecs.umich.edu/$\sim$panalyzer})] \newline

Os autores não utilizaram nenhum \textit{benchmark} específico. } \\ \hline \hline

\multicolumn{2}{|c|}{\textbf{Impacto (positivo x negativo)}} \\ \hline
\multicolumn{2}{|p{20cm}|}{O artigo apresentou como ponto positivo uma metodologia que aplica algoritmos genéticos para diminuição do consumo de energia em sisteam de tempo real. Como ponto negativo, a metodologia nem sempre consegue alcançar bons resultados de economia de energia, dependendo dos parâmetros iniciais das tarefas.} \\ \hline \hline

\multicolumn{2}{|c|}{\textbf{Validação do método}} \\ \hline
\multicolumn{2}{|p{20cm}|}{A validação da metodologia ocorreu pelo uso de de ferramentas e casos de teste definidos pelo próprio autor.} \\ \hline \hline

\multicolumn{2}{|c|}{\textbf{Limitações do método}} \\ \hline
\multicolumn{2}{|p{20cm}|}{O autor relata que em alguns casos é impossível alcançar frequências ideais no processador, caso contrário o deadline e outras restrições temporais podem ser violadas.} \\ \hline \hline

\multicolumn{2}{|c|}{\textbf{Integração de métodos}} \\ \hline
\multicolumn{2}{|p{20cm}|}{Integrou as técnica DVFS intra-task com a técnica DVFS inter-task.} \\ \hline \hline

\multicolumn{2}{|c|}{\textbf{Modo de aplicação do método}} \\ \hline
\multicolumn{2}{|p{20cm}|}{Híbrida} \\ \hline \hline

\multicolumn{2}{|c|}{\textbf{Perspectivas futuras}} \\ \hline
\multicolumn{2}{|p{20cm}|}{O autor propõe que os trabalhos futuros devem introduzir estimadores dinâmicos para a quantidade de ciclos de execução.} \\ \hline \hline

\multicolumn{2}{|c|}{\textbf{Comentários}} \\ \hline
\multicolumn{2}{|p{20cm}|}{A metodologia proposta não mostra evidências, no artigo, de que fornece suporte para recursos compartilhados e / ou preempções.} \\ \hline
\end{tabular}
}
\end{table}


%**********************************************************
% PUBLICACAO - ID_EXCEL: 157
%**********************************************************
\newpage
\begin{table}[htp] % h:here; t:top; b:bottom; p:page; default:ht
\centering
\caption{Dados extraído da publicação de \cite{Yi_Chen_Yang_2006_a}.}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{|p{3.8cm}|p{16cm}|}
\hline
\multicolumn{1}{|r|}{\textbf{ID}} & Yi\_Chen\_Yang\_2006\_a \\ \hline
\multicolumn{1}{|r|}{\textbf{Título}} & Static WCET analysis based compiler-directed DVS energy optimization in real-time applications \\ \hline
\multicolumn{1}{|r|}{\textbf{Autores}} & Yi H., Chen J., Yang X. \\ \hline
\multicolumn{1}{|r|}{\textbf{Palavras-chave}} & Compiler; Low-power; Real-time; WCET \\ \hline
\multicolumn{1}{|r|}{\textbf{Fonte da publicação}} & 11th Asia-Pacific Conference on Advances in Computer Systems Architecture, ACSAC 2006; \\ \hline
\multicolumn{1}{|r|}{\textbf{Editora}} & Springer \\ \hline
\multicolumn{1}{|r|}{\textbf{Ano da publicação}} & 2006 \\ \hline \hline

\multicolumn{2}{|c|}{\textbf{Resumo da publicação}} \\ \hline
\multicolumn{2}{|p{20cm}|}{Os autores propõem uma ferramenta chamada HEPTANE, cuja função é realizar a análise estática do WCET (em inglês, \textit{Worst Case Execution Time}), inserir os códigos da técnica DVFS e definir o perfil de consumo de energia da aplicação. Essa ferramenta trabalha em conjunto com o simulador de energia e performance chamado \textit{Sim-Panalyzer}, que roda em um ambiente \textit{RTLPower} (em inglês, \textit{Real-Time Low Power}), cuja função é simular o ambiente de experimentação para rodar os casos de teste criados pelos autores. Analisando de forma mais incisiva o trabalho, não ficou claro como a ferramenta HEPTANE trata as invariante de \textit{loops}, na definição do perfil de consumo de energia da aplicação.} \\ \hline \hline

\multicolumn{1}{|r|}{\textbf{Método(s) utilizados}} & DVFS Intra-Task; Control flow graph (CFG); \\ \hline
\multicolumn{1}{|r|}{\textbf{Ferramenta(s)}} & {O autor utilizou um ambiente nomeado de RTLPower (\textit{Real-Time Low Power}), que utiliza as seguintes ferramentas: \newline
- HEPTANE WCET \textit{analysis tool} [Enviar e-mail para puaut@irisa.fr solicitando a ferramenta]. \newline
- Sim-Panalyzer \textit{performance / power simulator} [Ferramenta não disponível para download - Site fora do ar (\href{http://www.eecs.umich.edu/~panalyzer}{http://www.eecs.umich.edu/$\sim$panalyzer})] \newline

Os \textit{benchmarks} utilizados foram: \newline
- SNU-RT \textit{benchmark} [Disponível em: \href{http://www.cprover.org/goto-cc/examples/snu.html}{http://www.cprover.org/goto-cc/examples/snu.html}] \newline
- \textit{Fast Fourier Transform} (fft1k) \newline
- \textit{Matrix Multiplication} (matmul)} \\ \hline \hline

\multicolumn{2}{|c|}{\textbf{Impacto (positivo x negativo)}} \\ \hline
\multicolumn{2}{|p{20cm}|}{O artigo apresentou como ponto positivo uma metodologia que realiza a análise estática do WCET (\textit{Worst Case Execution Time}) em aplicações de tempo real, uma vez que a maioria das soluções presentes na literatura leva em consideração o WCEC (\textit{Worst Case Execution Cycle}). Como ponto negativo, a metodologia não deixa claro como são feitas as análises de estruturas como \textit{loops} e \textit{loops} ocultos.} \\ \hline \hline

\multicolumn{2}{|c|}{\textbf{Validação do método}} \\ \hline
\multicolumn{2}{|p{20cm}|}{A validação da metodologia ocorreu pelo uso de de ferramentas e \textit{Benchmarks} relatados na literatura. Além disso, compara os resultados experimentais com outros trabalhos de referência na área de baixo consumo de energia.} \\ \hline \hline

\multicolumn{2}{|c|}{\textbf{Limitações do método}} \\ \hline
\multicolumn{2}{|p{20cm}|}{A metodologia não prever a análise estática de recursões.} \\ \hline \hline

\multicolumn{2}{|c|}{\textbf{Integração de métodos}} \\ \hline
\multicolumn{2}{|p{20cm}|}{Não se aplica} \\ \hline \hline

\multicolumn{2}{|c|}{\textbf{Modo de aplicação do método}} \\ \hline
\multicolumn{2}{|p{20cm}|}{Offline} \\ \hline \hline

\multicolumn{2}{|c|}{\textbf{Perspectivas futuras}} \\ \hline
\multicolumn{2}{|p{20cm}|}{O autor não relata nenhuma perspectiva futura. No entanto, poderiam ser adicionado análise estáticas para trabalhar com recursões.} \\ \hline \hline

\multicolumn{2}{|c|}{\textbf{Comentários}} \\ \hline
\multicolumn{2}{|p{20cm}|}{A metodologia proposta não mostra evidências, no artigo, de que fornece suporte para recursos compartilhados e / ou preempções.} \\ \hline
\end{tabular}
}
\end{table}


%**********************************************************
% PUBLICACAO - ID_EXCEL: 153
%**********************************************************
\newpage
\begin{table}[htp] % h:here; t:top; b:bottom; p:page; default:ht
\centering
\caption{Dados extraído da publicação de \cite{Shin_Kim_2007_a}.}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{|p{3.8cm}|p{16cm}|}
\hline
\multicolumn{1}{|r|}{\textbf{ID}} & Shin\_Kim\_2007\_a \\ \hline
\multicolumn{1}{|r|}{\textbf{Título}} & Optimizing intratask voltage scheduling using profile and data-flow information \\ \hline
\multicolumn{1}{|r|}{\textbf{Autores}} & Shin D., Kim J. \\ \hline
\multicolumn{1}{|r|}{\textbf{Palavras-chave}} & Dynamic-voltage scaling; Low-power design; Power management; Real-time systems; Variable-voltage processor \\ \hline
\multicolumn{1}{|r|}{\textbf{Fonte da publicação}} & IEEE Transactions on Computer-Aided Design of Integrated Circuits and Systems \\ \hline
\multicolumn{1}{|r|}{\textbf{Editora}} & IEEE \\ \hline
\multicolumn{1}{|r|}{\textbf{Ano da publicação}} & 2007 \\ \hline \hline

\multicolumn{2}{|c|}{\textbf{Resumo da publicação}} \\ \hline
\multicolumn{2}{|p{20cm}|}{Os autores propõem duas melhorias sobre a técnica IntraDVS. A primeira delas é uma melhoria da técnica chamada RAEP-IntraDVS (em inglês, \textit{Remaining Average-case Execution Path}), que visa otimizar o escalonamento de tensão através de análises das informações da aplicação, levando em consideração o caminho de execução de caso médio remanescente. A outra melhoria é sobre a técnica LaIntraDVS, citada no trabalho \cite{Shin_Kim_2005_b}, que leva em consideração as informações do fluxo de dados para gerar otimizações sobre os pontos de chaveamento de tensão (em inglês, \textit{Voltage-Scaling Points} - VSPs), principalmente através da predição das VSPs antes de estruturas condicionais e \textit{loops}.} \\ \hline \hline

\multicolumn{1}{|r|}{\textbf{Método(s) utilizados}} & DVFS Intra-Task; Control flow graph (CFG); \\ \hline
\multicolumn{1}{|r|}{\textbf{Ferramenta(s)}} & {Os autores não especificaram a ferramenta utilizada para a realização dos experimentos, mas deixou claro que utilizou o MPEG-4 \textit{encoder} como \textit{benchmark}.} \\ \hline \hline

\multicolumn{2}{|c|}{\textbf{Impacto (positivo x negativo)}} \\ \hline
\multicolumn{2}{|p{20cm}|}{O artigo apresentou como ponto positivo uma metodologia que reduz o overhead sobre a técnica DVS intra-tarefas através do melhor gerenciamento dos pontos de escalonamento de tensão. Como ponto negativo, a metodologia não claro como ela faz para definir VSPs diante de invariantes de \textit{loops}.} \\ \hline \hline

\multicolumn{2}{|c|}{\textbf{Validação do método}} \\ \hline
\multicolumn{2}{|p{20cm}|}{A validação da metodologia ocorreu pelo uso de \textit{Benchmark} presente na literatura. Além disso, compara os resultados experimentais com outros trabalhos de referência na área de baixo consumo de energia.} \\ \hline \hline

\multicolumn{2}{|c|}{\textbf{Limitações do método}} \\ \hline
\multicolumn{2}{|p{20cm}|}{A metodologia não deixou claro no artigo como faz para lhe dar com invariantes de \textit{loops} ao definir as VSPs.} \\ \hline \hline

\multicolumn{2}{|c|}{\textbf{Integração de métodos}} \\ \hline
\multicolumn{2}{|p{20cm}|}{Não se aplica} \\ \hline \hline

\multicolumn{2}{|c|}{\textbf{Modo de aplicação do método}} \\ \hline
\multicolumn{2}{|p{20cm}|}{Offline} \\ \hline \hline

\multicolumn{2}{|c|}{\textbf{Perspectivas futuras}} \\ \hline
\multicolumn{2}{|p{20cm}|}{O autor visa melhorar sua metodologia adicionando características para lhe dar com energia de fulga (\textit{leakage power}) e energia dinâmica (\textit{dynamic power}) do processador.} \\ \hline \hline

\multicolumn{2}{|c|}{\textbf{Comentários}} \\ \hline
\multicolumn{2}{|p{20cm}|}{A metodologia proposta não mostra evidências, no artigo, de que fornece suporte para recursos compartilhados e / ou preempções.} \\ \hline
\end{tabular}
}
\end{table}


%**********************************************************
% PUBLICACAO - ID_EXCEL: 147
%**********************************************************
\newpage
\begin{table}[htp] % h:here; t:top; b:bottom; p:page; default:ht
\centering
\caption{Dados extraído da publicação de \cite{Neishaburi_2007_a}.}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{|p{3.8cm}|p{16cm}|}
\hline
\multicolumn{1}{|r|}{\textbf{ID}} & Neishaburi\_2007\_a \\ \hline
\multicolumn{1}{|r|}{\textbf{Título}} & System level voltage scheduling technique using UML-RT model \\ \hline
\multicolumn{1}{|r|}{\textbf{Autores}} & Neishaburi M.H., Daneshtalab M., Nabi M., Mohammadi S. \\ \hline
\multicolumn{1}{|r|}{\textbf{Palavras-chave}} & Intra-task voltage scheduling; JPEG encoder system; System level voltage scheduling; UML-RT model; Data flow analysis; Data transfer; Encoding (symbols); Energy utilization; Voltage control; Scheduling algorithms \\ \hline
\multicolumn{1}{|r|}{\textbf{Fonte da publicação}} & 2007 IEEE/ACS International Conference on Computer Systems and Applications, AICCSA 2007 \\ \hline
\multicolumn{1}{|r|}{\textbf{Editora}} & IEEE \\ \hline
\multicolumn{1}{|r|}{\textbf{Ano da publicação}} & 2007 \\ \hline \hline

\multicolumn{2}{|c|}{\textbf{Resumo da publicação}} \\ \hline
\multicolumn{2}{|p{20cm}|}{Os autores apresentam uma otimização sobre o escalonamento de tensões intra-tarefa, através da análise do fluxo de dados e do fluxo de controle da aplicação. A partir dessa análise, a metodologia é capaz de antecipar os pontos de escalonamento de tensão (em inglês, \textit{Voltage Scaling Points} - VSP), enquanto que a técnica DVFS intra-tarefa tradicional apenas localiza os pontos de controle. Essa metodologia permite adicionar menos \textit{overheads} no código fonte da aplicação.} \\ \hline \hline

\multicolumn{1}{|r|}{\textbf{Método(s) utilizados}} & DVFS Intra-Task; Control flow graph (CFG); \\ \hline
\multicolumn{1}{|r|}{\textbf{Ferramenta(s)}} & {Os autores utilizaram a ferramenta UML-RT e o JPEG \textit{encoder} como \textit{benchmark}.} \\ \hline \hline

\multicolumn{2}{|c|}{\textbf{Impacto (positivo x negativo)}} \\ \hline
\multicolumn{2}{|p{20cm}|}{O artigo apresentou como ponto positivo uma metodologia propõe uma nova forma de analisar os grafos de fluxo de controle da aplicação a fim de diminuir os \textit{overheads} inseridos dentro das tarefas. Como ponto negativo, a metodologia tem dificuldade para lhe dar alguns tipos de estruturas, como: \textit{loops} e recursões.} \\ \hline \hline

\multicolumn{2}{|c|}{\textbf{Validação do método}} \\ \hline
\multicolumn{2}{|p{20cm}|}{A validação da metodologia ocorreu pelo uso de ferramenta e \textit{Benchmark} presentes na literatura.} \\ \hline \hline

\multicolumn{2}{|c|}{\textbf{Limitações do método}} \\ \hline
\multicolumn{2}{|p{20cm}|}{A metodologia possui dificuldade para lhe dar com funções recursivas (profundidade desconhecida), volta de saltos incondicionais (\textit{loops} ocultos) e chamadas de funções dinâmicas.} \\ \hline \hline

\multicolumn{2}{|c|}{\textbf{Integração de métodos}} \\ \hline
\multicolumn{2}{|p{20cm}|}{Não se aplica} \\ \hline \hline

\multicolumn{2}{|c|}{\textbf{Modo de aplicação do método}} \\ \hline
\multicolumn{2}{|p{20cm}|}{Offline} \\ \hline \hline

\multicolumn{2}{|c|}{\textbf{Perspectivas futuras}} \\ \hline
\multicolumn{2}{|p{20cm}|}{Melhor a metodologia para lhe dar melhor com loops e chamadas recursivas.} \\ \hline \hline

\multicolumn{2}{|c|}{\textbf{Comentários}} \\ \hline
\multicolumn{2}{|p{20cm}|}{A metodologia proposta não mostra evidências, no artigo, de que fornece suporte para recursos compartilhados e/ou preempções.} \\ \hline
\end{tabular}
}
\end{table}


%**********************************************************
% PUBLICACAO - ID_EXCEL: 124
%**********************************************************
\newpage
\begin{table}[htp] % h:here; t:top; b:bottom; p:page; default:ht
\centering
\caption{Dados extraído da publicação de \cite{Chen_Hsieh_Lai_2008_b}.}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{|p{3.8cm}|p{16cm}|}
\hline
\multicolumn{1}{|r|}{\textbf{ID}} & Chen\_Hsieh\_Lai\_2008\_b \\ \hline
\multicolumn{1}{|r|}{\textbf{Título}} & Efficient algorithms for periodic real-time tasks to optimal discrete voltage schedules \\ \hline
\multicolumn{1}{|r|}{\textbf{Autores}} & Chen D.-R., Hsieh S.-M., Lai M.-F. \\ \hline
\multicolumn{1}{|r|}{\textbf{Palavras-chave}} & Dynamic voltage scaling; Hard real-time systems; Jitter control; Power-aware scheduling \\ \hline
\multicolumn{1}{|r|}{\textbf{Fonte da publicação}} & IPDPS Miami 2008 - Proceedings of the 22nd IEEE International Parallel and Distributed Processing Symposium, Program and CD-ROM \\ \hline
\multicolumn{1}{|r|}{\textbf{Editora}} & IEEE \\ \hline
\multicolumn{1}{|r|}{\textbf{Ano da publicação}} & 2008 \\ \hline \hline

\multicolumn{2}{|c|}{\textbf{Resumo da publicação}} \\ \hline
\multicolumn{2}{|p{20cm}|}{Os autores propõem uma metodologia que visa minimizar o consumo de energia através da análise do fluxo de dados da aplicação, tanto do ponto de vista inter quanto intra tarefa. Essa abordagem consiste basicamente de três fases: (1) primeiramente é feita a transformação harmônica dos períodos de todas as tarefas, em seguida é feita a validação e compartilhamento dos tempo de folga entre as demais tarefas, utilizando um escalonamento definidos pelos autores de \textit{Jitterless Schedule}, que são interferências causadas pela chegada de sucessivas instâncias de uma mesma tarefa.; (2) o próximo passo é calcular a utilização total dado os novos parâmetros das tarefas definidos no passo 1; por último (3) é feita a computação das características de cada tarefa, tais como o início e fim relativos, com o objetivo de ajustar as tensões e frequência, evitando que restrições temporais venham ser violadas. } \\ \hline \hline

\multicolumn{1}{|r|}{\textbf{Método(s) utilizados}} & DVFS Intra-Task; DVFS Inter-Task; \\ \hline
\multicolumn{1}{|r|}{\textbf{Ferramenta(s)}} & {Os autores não especificaram a ferramenta utilizada para a realização dos experimentos e não utilizou nenhum \textit{benchmark}.} \\ \hline \hline

\multicolumn{2}{|c|}{\textbf{Impacto (positivo x negativo)}} \\ \hline
\multicolumn{2}{|p{20cm}|}{O artigo apresentou como ponto positivo uma metodologia que propõe um escalonamento de tarefas com menor \textit{jitter}. Como ponto negativo, os autores não aplicam nenhum Benchmark para avaliação dos reais ganhos da metodologia proposta.} \\ \hline \hline

\multicolumn{2}{|c|}{\textbf{Validação do método}} \\ \hline
\multicolumn{2}{|p{20cm}|}{A validação da metodologia ocorreu pelo uso de provas formais e comparações de desempenho de complexidade computacional com outros trabalhos presentes na literatura.} \\ \hline \hline

\multicolumn{2}{|c|}{\textbf{Limitações do método}} \\ \hline
\multicolumn{2}{|p{20cm}|}{Os autores não deixam claro sobre os overheads ocasionados pelo uso de sua metodologia.} \\ \hline \hline

\multicolumn{2}{|c|}{\textbf{Integração de métodos}} \\ \hline
\multicolumn{2}{|p{20cm}|}{Integrou as técnicas DVFS intra-tarefa com a técnica DVFS inter-tarefa} \\ \hline \hline

\multicolumn{2}{|c|}{\textbf{Modo de aplicação do método}} \\ \hline
\multicolumn{2}{|p{20cm}|}{Offline} \\ \hline \hline

\multicolumn{2}{|c|}{\textbf{Perspectivas futuras}} \\ \hline
\multicolumn{2}{|p{20cm}|}{Não identificada diretamente} \\ \hline \hline

\multicolumn{2}{|c|}{\textbf{Comentários}} \\ \hline
\multicolumn{2}{|p{20cm}|}{A metodologia proposta não mostra evidências, no artigo, de que fornece suporte para recursos compartilhados e / ou preempções.} \\ \hline
\end{tabular}
}
\end{table}


%**********************************************************
% PUBLICACAO - ID_EXCEL: 122
%**********************************************************
\newpage
\begin{table}[htp] % h:here; t:top; b:bottom; p:page; default:ht
\centering
\caption{Dados extraído da publicação de \cite{Oh_Kim_Kim_Kyung_2008_a}.}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{|p{3.8cm}|p{16cm}|}
\hline
\multicolumn{1}{|r|}{\textbf{ID}} & Oh\_Kim\_Kim\_Kyung\_2008\_a \\ \hline
\multicolumn{1}{|r|}{\textbf{Título}} & Task partitioning algorithm for intra-task dynamic voltage scaling \\ \hline
\multicolumn{1}{|r|}{\textbf{Autores}} & Oh S., Kim J., Kim S., Kyung C.-M. \\ \hline
\multicolumn{1}{|r|}{\textbf{Palavras-chave}} & Dynamic voltage scaling; International symposium; Voltage switching; Axial flow; Boolean functions; Electric load forecasting; Technical presentations; Electric network analysis \\ \hline
\multicolumn{1}{|r|}{\textbf{Fonte da publicação}} & Proceedings - IEEE International Symposium on Circuits and Systems \\ \hline
\multicolumn{1}{|r|}{\textbf{Editora}} & IEEE \\ \hline
\multicolumn{1}{|r|}{\textbf{Ano da publicação}} & 2008 \\ \hline \hline

\multicolumn{2}{|c|}{\textbf{Resumo da publicação}} \\ \hline
\multicolumn{2}{|p{20cm}|}{Os autores propõem um novo algoritmo de particionamento de tarefas baseado na técnica DVS intra-tarefa, onde o seu principal objetivo é dividir de maneira mais eficiente os blocos de código da aplicação de forma que seja possível diminuir o número de chaveamento de tensões e frequências do processador. Essa abordagem, primeiramente, divide o código fonte da aplicação em um número máximo de seções de código. Em seguida, são calculados os ciclos de execução de cada nó, por meio de simulações estáticas, e as penalidades das predições que falharam. Essas penalidades são utilizadas como uma medida para decidir se determinados nós deverão ser agrupados ou não. Com essa metodologia os autores conseguiram reduzir o número de chaveamentos de tensão e, consequentemente, minimizar o consumo de energia do processador.} \\ \hline \hline

\multicolumn{1}{|r|}{\textbf{Método(s) utilizados}} & DVFS Intra-Task; \\ \hline
\multicolumn{1}{|r|}{\textbf{Ferramenta(s)}} & {Os autores não especificaram a ferramenta utilizada para a realização dos experimentos, somente o \textit{hardware} utilizado. \newline

Os autores utilizaram o \textit{benchmark}: \newline
- H.264 \textit{Decoder} } \\ \hline \hline

\multicolumn{2}{|c|}{\textbf{Impacto (positivo x negativo)}} \\ \hline
\multicolumn{2}{|p{20cm}|}{O artigo apresentou como ponto positivo uma metodologia para analisar a divisão eficiente dos blocos de código de uma aplicação. Como ponto negativo, os autores não leva em consideração as preempções durante a realização dos experimentos. } \\ \hline \hline

\multicolumn{2}{|c|}{\textbf{Validação do método}} \\ \hline
\multicolumn{2}{|p{20cm}|}{A validação da metodologia ocorreu pelo uso de \textit{Benchmark} presente na literatura. Além disso, compara os resultados experimentais com outros trabalhos de referência na área de baixo consumo de energia.} \\ \hline \hline

\multicolumn{2}{|c|}{\textbf{Limitações do método}} \\ \hline
\multicolumn{2}{|p{20cm}|}{O metodologia apresentada não leva em consideração as preempções.} \\ \hline \hline

\multicolumn{2}{|c|}{\textbf{Integração de métodos}} \\ \hline
\multicolumn{2}{|p{20cm}|}{Não se aplica.} \\ \hline \hline

\multicolumn{2}{|c|}{\textbf{Modo de aplicação do método}} \\ \hline
\multicolumn{2}{|p{20cm}|}{Offline} \\ \hline \hline

\multicolumn{2}{|c|}{\textbf{Perspectivas futuras}} \\ \hline
\multicolumn{2}{|p{20cm}|}{Não identificada diretamente} \\ \hline \hline

\multicolumn{2}{|c|}{\textbf{Comentários}} \\ \hline
\multicolumn{2}{|p{20cm}|}{A metodologia proposta não mostra evidências, no artigo, de que fornece suporte para recursos compartilhados e / ou preempções.} \\ \hline
\end{tabular}
}
\end{table}


%**********************************************************
% PUBLICACAO - ID_EXCEL: 113
%**********************************************************
\newpage
\begin{table}[htp] % h:here; t:top; b:bottom; p:page; default:ht
\centering
\caption{Dados extraído da publicação de \cite{Zitterell_2008_a}.}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{|p{3.8cm}|p{16cm}|}
\hline
\multicolumn{1}{|r|}{\textbf{ID}} & Zitterell\_2008\_a \\ \hline
\multicolumn{1}{|r|}{\textbf{Título}} & Improving energy-efficient real-time scheduling by exploiting code instrumentation \\ \hline
\multicolumn{1}{|r|}{\textbf{Autores}} & Zitterell T., Scholl C. \\ \hline
\multicolumn{1}{|r|}{\textbf{Palavras-chave}} & Code instrumentation; Discrete frequencies; Dynamic frequency; Energy efficient; Frequency-scaling; Idle time; Library functions; Light weight; Low frequency; Real time scheduling; Save energy; Simulation framework; Slack time; Task information; Task-scheduling; Voltage-scaling; Computer science; Energy efficiency; Information technology; Program compilers; Response time (computer systems); Scheduling; Real time systems \\ \hline
\multicolumn{1}{|r|}{\textbf{Fonte da publicação}} & Proceedings of the International Multiconference on Computer Science and Information Technology, IMCSIT 2008 \\ \hline
\multicolumn{1}{|r|}{\textbf{Editora}} & IEEE \\ \hline
\multicolumn{1}{|r|}{\textbf{Ano da publicação}} & 2008 \\ \hline \hline

\multicolumn{2}{|c|}{\textbf{Resumo da publicação}} \\ \hline
\multicolumn{2}{|p{20cm}|}{Os autores propõem um escalonamento mais eficiente de energia para processadores com frequências discretas, chamado de ItcaEDF (em inglês, \textit{Intra-Task Characteristics Aware EDF}). Ela se baseia na integração das técnicas inter e intra tarefas para diminuição dos tempos ociosos do processador e dos tempos de folgas das tarefas. No algoritmo intra-tarefa, os autores focam na quantidade de ciclos economizados e em um contador de ciclos, que possibilita contabilizar os diferentes caminhos dentro de um \textit{loop}, permitindo diminuir os níveis de frequência do processador de acordo com as invariantes do \textit{loop}. Quanto ao algoritmo inter-tarefa, os autores implementam um conjunto de bibliotecas que permitem as tarefas compartilhar informações umas com as outras, contribuindo para um melhor escalonamento global e diminuição do tempo ocioso do processador.} \\ \hline \hline

\multicolumn{1}{|r|}{\textbf{Método(s) utilizados}} & DVFS Intra-Task; DVFS Inter-Task; Control Flow Graph (CFG); \\ \hline
\multicolumn{1}{|r|}{\textbf{Ferramenta(s)}} & {O autor não especificou a ferramenta utilizada para a realização dos experimentos.} \\ \hline \hline

\multicolumn{2}{|c|}{\textbf{Impacto (positivo x negativo)}} \\ \hline
\multicolumn{2}{|p{20cm}|}{O artigo apresentou como ponto positivo uma metodologia que explora invariantes de \textit{loops} para realizar o melhor controle da quantidade de ciclos a serem executados. Como ponto negativo, os autores não deixam claro no artigo os reais impactos gerados pelo uso da sua metodologia, principalmente do ponto de visto dos overhead, uma vez que a solução proposta é uma abordagem \textit{online}.} \\ \hline \hline

\multicolumn{2}{|c|}{\textbf{Validação do método}} \\ \hline
\multicolumn{2}{|p{20cm}|}{A validação da metodologia ocorreu pelo uso de casos de teste gerados pelo próprio autor. No entanto, os resultados experimentais são comparados com outras abordagens presentes na literatura.} \\ \hline \hline

\multicolumn{2}{|c|}{\textbf{Limitações do método}} \\ \hline
\multicolumn{2}{|p{20cm}|}{O método não deixa claro sobre os \textit{overheads} gerados pelas inclusões das bibliotecas de compartilhamento de dados entre tarefas em execução.} \\ \hline \hline

\multicolumn{2}{|c|}{\textbf{Integração de métodos}} \\ \hline
\multicolumn{2}{|p{20cm}|}{Integrou a técnica DVFS intra-tarefas com a técnica DVFS inter-tarefa} \\ \hline \hline

\multicolumn{2}{|c|}{\textbf{Modo de aplicação do método}} \\ \hline
\multicolumn{2}{|p{20cm}|}{Online} \\ \hline \hline

\multicolumn{2}{|c|}{\textbf{Perspectivas futuras}} \\ \hline
\multicolumn{2}{|p{20cm}|}{Fazer um estudo mais detalhados sobre os \textit{overheads} gerados pela aplicação da metodologia proposta.} \\ \hline \hline

\multicolumn{2}{|c|}{\textbf{Comentários}} \\ \hline
\multicolumn{2}{|p{20cm}|}{A metodologia proposta não mostra evidências, no artigo, de que fornece suporte para recursos compartilhados e / ou preempções.} \\ \hline
\end{tabular}
}
\end{table}


%**********************************************************
% PUBLICACAO - ID_EXCEL: 112
%**********************************************************
\newpage
\begin{table}[htp] % h:here; t:top; b:bottom; p:page; default:ht
\centering
\caption{Dados extraído da publicação de \cite{Chen_2008_a}.}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{|p{3.8cm}|p{16cm}|}
\hline
\multicolumn{1}{|r|}{\textbf{ID}} & Chen\_2008\_a \\ \hline
\multicolumn{1}{|r|}{\textbf{Título}} & Expected energy consumption minimization in DVS systems with discrete frequencies \\ \hline
\multicolumn{1}{|r|}{\textbf{Autores}} & Chen J.-J. \\ \hline
\multicolumn{1}{|r|}{\textbf{Palavras-chave}} & Dynamic voltage scaling; Energy-efficient scheduling; Expected energy consumption minimization; Probability \\ \hline
\multicolumn{1}{|r|}{\textbf{Fonte da publicação}} & Proceedings of the ACM Symposium on Applied Computing \\ \hline
\multicolumn{1}{|r|}{\textbf{Editora}} & ACM \\ \hline
\multicolumn{1}{|r|}{\textbf{Ano da publicação}} & 2008 \\ \hline \hline

\multicolumn{2}{|c|}{\textbf{Resumo da publicação}} \\ \hline
\multicolumn{2}{|p{20cm}|}{O autor apresenta uma nova abordagem para minimizar o consumo de energia utilizando funções de densidade de probabilidade com base nas cargas de trabalho das tarefas de tempo real. Para o escalonamento intra-tarefa foi feito um algoritmo eficiente para obter a frequência ideal para uma única tarefa, de modo que o consumo de energia seja minimizado. Enquanto que o algoritmo de escalonamento inter-tarefa, chamado \textit{M-Greedy}, foi desenvolvido com base em uma abordagem de programação linear cuja finalidade é obter as melhores soluções para as tarefas de tempo real baseada em quadros, visando diminuir os tempos de folga.} \\ \hline \hline

\multicolumn{1}{|r|}{\textbf{Método(s) utilizados}} & DVFS Intra-Task; DVFS Inter-Task; \\ \hline
\multicolumn{1}{|r|}{\textbf{Ferramenta(s)}} & {O autor não utilizou nenhuma ferramenta específica. No entanto, o autor utilizou os \textit{benchmarks}: \newline
- mpegplay (MPEG \textit{video decoder}) \newline
- madplay (MP3 \textit{audio decoder}) \newline
- tmndec (H.263 \textit{video decoder}) \newline
- toast (GSM \textit{speech encoder})} \\ \hline \hline

\multicolumn{2}{|c|}{\textbf{Impacto (positivo x negativo)}} \\ \hline
\multicolumn{2}{|p{20cm}|}{O artigo apresentou como ponto positivo uma metodologia para identificar a frequência ideal que uma tarefa deve executar para que haja baixo consumo de energia, sempre respeitando suas restrições temporais. Como ponto negativo, o autor leva em consideração uma única tarefa na aplicação da sua metodologia offline.} \\ \hline \hline

\multicolumn{2}{|c|}{\textbf{Validação do método}} \\ \hline
\multicolumn{2}{|p{20cm}|}{A validação da metodologia ocorreu através do uso de \textit{Benchmarks} relatados na literatura. Além disso, compara os resultados experimentais com outros trabalhos de referência na área de baixo consumo de energia.} \\ \hline \hline

\multicolumn{2}{|c|}{\textbf{Limitações do método}} \\ \hline
\multicolumn{2}{|p{20cm}|}{O algoritmo intra-tarefa leva em consideração apenas uma única tarefa.} \\ \hline \hline

\multicolumn{2}{|c|}{\textbf{Integração de métodos}} \\ \hline
\multicolumn{2}{|p{20cm}|}{Integrou a técnica DVFS intra-tarefas com a técnica DVFS inter-tarefa} \\ \hline \hline

\multicolumn{2}{|c|}{\textbf{Modo de aplicação do método}} \\ \hline
\multicolumn{2}{|p{20cm}|}{Híbrida} \\ \hline \hline

\multicolumn{2}{|c|}{\textbf{Perspectivas futuras}} \\ \hline
\multicolumn{2}{|p{20cm}|}{Como perspectivas futuras, expandir a metodologia proposta para outros dispositivos periféricos (perspectiva sugerida pelo próprio autor).} \\ \hline \hline

\multicolumn{2}{|c|}{\textbf{Comentários}} \\ \hline
\multicolumn{2}{|p{20cm}|}{A artigo comenta que as tarefas podem ser preemptadas por outras de maior prioridade, mas não deixa claro como é feito esse tratamento. Quanto aos recursos compartilhados, a metodologia não dá suporte.} \\ \hline
\end{tabular}
}
\end{table}


%**********************************************************
% PUBLICACAO - ID_EXCEL: 110
%**********************************************************
\newpage
\begin{table}[htp] % h:here; t:top; b:bottom; p:page; default:ht
\centering
\caption{Dados extraído da publicação de \cite{Chen_Hsieh_Lai_2008_a}.}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{|p{3.8cm}|p{16cm}|}
\hline
\multicolumn{1}{|r|}{\textbf{ID}} & Chen\_Hsieh\_Lai\_2008\_a \\ \hline
\multicolumn{1}{|r|}{\textbf{Título}} & Efficient algorithms for jitterless real-time tasks to DVS schedules \\ \hline
\multicolumn{1}{|r|}{\textbf{Autores}} & Chen D.-R., Hsieh S.-M., Lai M.-F. \\ \hline
\multicolumn{1}{|r|}{\textbf{Palavras-chave}} & Canonical schedules; Dvs algorithms; DVS schedules; Efficient algorithms; Finish times; Minimum energies; Periodic tasks; Real-time tasks; Variable voltages; Voltage stabilizing circuits \\ \hline
\multicolumn{1}{|r|}{\textbf{Fonte da publicação}} & Parallel and Distributed Computing, Applications and Technologies, PDCAT Proceedings \\ \hline
\multicolumn{1}{|r|}{\textbf{Editora}} & IEEE \\ \hline
\multicolumn{1}{|r|}{\textbf{Ano da publicação}} & 2008 \\ \hline \hline

\multicolumn{2}{|c|}{\textbf{Resumo da publicação}} \\ \hline
\multicolumn{2}{|p{20cm}|}{Os autores propõem um algoritmo intra-tarefa e um inter-tarefa para diminuir o consumo de energia durante o escalonamento das tarefas. Essa metodologia tem como finalidade diminuir os \textit{overheads} e os tempos de folga entre as tarefas, dando mais previsibilidade e otimizações \textit{offline} para o escalonamento. Para facilitar a geração do escalonamento, as tarefas com períodos arbitrários são transformados em períodos harmônicos para que os tempos de preempção, início e término de cada tarefa possam ser facilmente derivados, principalmente para tratar o que o autor chama de \textit{Jitterless Schedule}. Essa abordagem foi desenvolvida a partir do trabalho de \cite{Chen_Hsieh_Lai_2008_b}.} \\ \hline \hline

\multicolumn{1}{|r|}{\textbf{Método(s) utilizados}} & DVFS Intra-Task; DVFS Inter-Task; \\ \hline
\multicolumn{1}{|r|}{\textbf{Ferramenta(s)}} & {Os autores não utilizaram nenhuma ferramenta ou benchmark.} \\ \hline \hline

\multicolumn{2}{|c|}{\textbf{Impacto (positivo x negativo)}} \\ \hline
\multicolumn{2}{|p{20cm}|}{O artigo apresentou como ponto positivo uma metodologia para lidar com preempções e interferências entre tarefas. Como ponto negativo, os autores não utilizaram nenhum \textit{benchmark} para a realização dos seus experimentos. } \\ \hline \hline

\multicolumn{2}{|c|}{\textbf{Validação do método}} \\ \hline
\multicolumn{2}{|p{20cm}|}{A validação da metodologia ocorreu pelo uso de casos de testes gerados pelos próprios autores. No entanto, os resultados experimentais são comparados com outras abordagens presentes na literatura.} \\ \hline \hline

\multicolumn{2}{|c|}{\textbf{Limitações do método}} \\ \hline
\multicolumn{2}{|p{20cm}|}{Faltou aplicar \textit{benchmarks} na realização dos experimentos.} \\ \hline \hline

\multicolumn{2}{|c|}{\textbf{Integração de métodos}} \\ \hline
\multicolumn{2}{|p{20cm}|}{Integrou a técnica DVFS intra-tarefas com a técnica DVFS inter-tarefa} \\ \hline \hline

\multicolumn{2}{|c|}{\textbf{Modo de aplicação do método}} \\ \hline
\multicolumn{2}{|p{20cm}|}{Offline} \\ \hline \hline

\multicolumn{2}{|c|}{\textbf{Perspectivas futuras}} \\ \hline
\multicolumn{2}{|p{20cm}|}{Não identificada diretamente} \\ \hline \hline

\multicolumn{2}{|c|}{\textbf{Comentários}} \\ \hline
\multicolumn{2}{|p{20cm}|}{
- O autor apresentou apenas comparações de complexidade em relação a alguns trabalhos da literatura. Faltou mostrar o real ganho da metodologia apresentada em níveis de consumo de energia.
- A metodologia proposta não mostra evidências, no artigo, de que fornece suporte para recursos compartilhados e / ou preempções.} \\ \hline
\end{tabular}
}
\end{table}


%**********************************************************
% PUBLICACAO - ID_EXCEL: 105
%**********************************************************
\newpage
\begin{table}[htp] % h:here; t:top; b:bottom; p:page; default:ht
\centering
\caption{Dados extraído da publicação de \cite{He_2008_a}.}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{|p{3.8cm}|p{16cm}|}
\hline
\multicolumn{1}{|r|}{\textbf{ID}} & He\_2008\_a \\ \hline
\multicolumn{1}{|r|}{\textbf{Título}} & Stochastic voltage scheduling of fixed-priority tasks with preemption thresholds \\ \hline
\multicolumn{1}{|r|}{\textbf{Autores}} & He X., Jia Y., Wa H. \\ \hline
\multicolumn{1}{|r|}{\textbf{Palavras-chave}} & Embedded systems; Energy management; Energy policy; Integrated circuits; Mobile computing; Scheduling; Voltage stabilizing circuits; Wireless networks; Wireless telecommunication systems; Clock speeds; Dynamic voltage scaling; Energy consumptions; Energy gains; Power managements; Preemption thresholds; Priority tasks; Responsiveness.; Scarce resources; Scheduling policies; Stochastic datums; Supply voltages; Variable execution times; Voltage scheduling; Real time systems \\ \hline
\multicolumn{1}{|r|}{\textbf{Fonte da publicação}} & 2008 International Conference on Wireless Communications, Networking and Mobile Computing, WiCOM 2008 \\ \hline
\multicolumn{1}{|r|}{\textbf{Editora}} & IEEE \\ \hline
\multicolumn{1}{|r|}{\textbf{Ano da publicação}} & 2008 \\ \hline \hline

\multicolumn{2}{|c|}{\textbf{Resumo da publicação}} \\ \hline
\multicolumn{2}{|p{20cm}|}{Os autores exploram os tempos de execução variáveis de tarefas, dentro da política de escalonamento FPPT (em inglês, \textit{Fixed-Priority scheduling with Preemption Threshold} - Escalonamento com Prioridade Fixa com Limite de Preempção). Essa política de escalonamento, executando em um processador com tensão variável, permite reduzir os custos com preempções desnecessárias das tarefas. Então, os autores desenvolveram um algoritmo para analisar todas as possibilidades de carga de trabalho para cada tarefa. Em seguida, utilizou esses dados estocásticos para definir as tensões e frequências do processador de acordo com o tamanho da tarefa e sua distribuição de probabilidade, com o intuito de minimizar o consumo de energia no caso médio.} \\ \hline \hline

\multicolumn{1}{|r|}{\textbf{Método(s) utilizados}} & DVFS Intra-Task; FPPT scheduling policy; \\ \hline
\multicolumn{1}{|r|}{\textbf{Ferramenta(s)}} & {Os autores utilizaram a ferramenta SPAK-0.3 (Disponível em: \href{http://www.cs.utah.edu/~regehr/spak/}{http://www.cs.utah.edu/$\sim$regehr/spak/}).} \\ \hline \hline

\multicolumn{2}{|c|}{\textbf{Impacto (positivo x negativo)}} \\ \hline
\multicolumn{2}{|p{20cm}|}{O artigo apresentou como ponto positivo uma metodologia que visa otimizar custos com preempções. Como ponto negativo, os autores deveriam aplicar algum \textit{benchmark} para a realização dos seus experimentos.} \\ \hline \hline

\multicolumn{2}{|c|}{\textbf{Validação do método}} \\ \hline
\multicolumn{2}{|p{20cm}|}{A validação da metodologia ocorreu pelo uso de ferramentas de simulação e de casos de testes gerados pelos próprios autores.} \\ \hline \hline

\multicolumn{2}{|c|}{\textbf{Limitações do método}} \\ \hline
\multicolumn{2}{|p{20cm}|}{A metodologia proposta não deixa muito claro como é feito o tratamento de preempção entre as tarefas em execução.} \\ \hline \hline

\multicolumn{2}{|c|}{\textbf{Integração de métodos}} \\ \hline
\multicolumn{2}{|p{20cm}|}{Integrou a política de escalonamento FPPT com a técnica DVFS intra-tarefa;} \\ \hline \hline

\multicolumn{2}{|c|}{\textbf{Modo de aplicação do método}} \\ \hline
\multicolumn{2}{|p{20cm}|}{Offline} \\ \hline \hline

\multicolumn{2}{|c|}{\textbf{Perspectivas futuras}} \\ \hline
\multicolumn{2}{|p{20cm}|}{Como perspectivas futuras, aplicar essa metodologia em algum RTOS (\textit{Real Time Operating System}).} \\ \hline \hline

\multicolumn{2}{|c|}{\textbf{Comentários}} \\ \hline
\multicolumn{2}{|p{20cm}|}{A metodologia proposta mostra indícios de que dá suporte a preempções, mas não fica muito claro no artigo como ela é feita. Quanto a recursos compartilhados, a metodologia não dá suporte.} \\ \hline
\end{tabular}
}
\end{table}


%**********************************************************
% PUBLICACAO - ID_EXCEL: 101
%**********************************************************
\newpage
\begin{table}[htp] % h:here; t:top; b:bottom; p:page; default:ht
\centering
\caption{Dados extraído da publicação de \cite{Yang_2009_a}.}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{|p{3.8cm}|p{16cm}|}
\hline
\multicolumn{1}{|r|}{\textbf{ID}} & Yang\_2009\_a \\ \hline
\multicolumn{1}{|r|}{\textbf{Título}} & Energy efficient intra-task dynamic voltage scaling for realistic CPUs of mobile devices \\ \hline
\multicolumn{1}{|r|}{\textbf{Autores}} & Yang C.-C., Wang K., Lin M.-H., Lin P. \\ \hline
\multicolumn{1}{|r|}{\textbf{Palavras-chave}} & CPU; Dynamic voltage scaling; Energy efficient; Intra-task; Mobile device; Real time \\ \hline
\multicolumn{1}{|r|}{\textbf{Fonte da publicação}} & Journal of Information Science and Engineering \\ \hline
\multicolumn{1}{|r|}{\textbf{Editora}} & Scopus (Elsevier) \\ \hline
\multicolumn{1}{|r|}{\textbf{Ano da publicação}} & 2009 \\ \hline \hline

\multicolumn{2}{|c|}{\textbf{Resumo da publicação}} \\ \hline
\multicolumn{2}{|p{20cm}|}{Os autores propõem dois algoritmos de escalonamento dinâmico de tensão (DVS) intra-tarefa para CPU's. O algoritmo OSRC (em inglês, \textit{Optimal Schedule for Realistic CPUs}) tem por objetivo aplicar conceitos de programação dinâmica dentro da CFG da aplicação para identificar os caminhos ideais com menor consumo de energia, tendo como referência a especificação de uma \textit{CPU} realista, que são processadores que possuem um conjunto limitado de níveis de tensão e frequência \citep{Yang_2009_a}. O segundo algoritmo, chamado LO-OSRC (em inglês, \textit{Low Overhead Optimal Schedule for Realistic CPUs}), já leva em consideração o potencial de computação das tarefas e os \textit{overheads} de transição, permitindo apenas uma mudanção de tensão de frequência da CPU por tarefa. Dessa forma, os autores mostram em seus experimentos que seus algoritmos conseguem obter ganhos acima de 10\% em comparação com outros trabalhos presentes na literatura.} \\ \hline \hline

\multicolumn{1}{|r|}{\textbf{Método(s) utilizados}} & DVFS Intra-Task; Control Flow Graph (CFG); Stochastic Method; \\ \hline
\multicolumn{1}{|r|}{\textbf{Ferramenta(s)}} & {Os autores específicam os \textit{hardwares} utilizados, mas não deixa claro as ferramentas ou softwares utilizados no experimentos e nem faz referência quanto ao uso de algum \textit{Benchmark}; } \\ \hline \hline

\multicolumn{2}{|c|}{\textbf{Impacto (positivo x negativo)}} \\ \hline
\multicolumn{2}{|p{20cm}|}{O artigo apresentou como ponto positivo a integração de métodos estocásticos a técnica DVFS intra-tarefa. Como ponto negativo, o autor utilizou somente dois modelos de tarefas para validar o seu método, onde o correto deveria ser utilizar várias modelos de tarefas diferentes visto que sua metodologia se basea em processos não determinísticos (ou seja, métodos estocásticos).} \\ \hline \hline

\multicolumn{2}{|c|}{\textbf{Validação do método}} \\ \hline
\multicolumn{2}{|p{20cm}|}{A validação da metodologia ocorreu pelo uso de casos de testes gerados pelo próprio autor e, além disso, compara os resultados experimentais obtidos com outras abordagens presentes na literatura.} \\ \hline \hline

\multicolumn{2}{|c|}{\textbf{Limitações do método}} \\ \hline
\multicolumn{2}{|p{20cm}|}{Os resultados foram gerados levando em consideração apenas dois modelos de tarefas e não levou em consideração preempções.} \\ \hline \hline

\multicolumn{2}{|c|}{\textbf{Integração de métodos}} \\ \hline
\multicolumn{2}{|p{20cm}|}{Integrou métodos estocásticos com a técnica DVFS intra-tarefa;} \\ \hline \hline

\multicolumn{2}{|c|}{\textbf{Modo de aplicação do método}} \\ \hline
\multicolumn{2}{|p{20cm}|}{Offline} \\ \hline \hline

\multicolumn{2}{|c|}{\textbf{Perspectivas futuras}} \\ \hline
\multicolumn{2}{|p{20cm}|}{Como perspectivas futuras, aplicar mais casos de testes para avaliar o real ganho da metodologia proposta.} \\ \hline \hline

\multicolumn{2}{|c|}{\textbf{Comentários}} \\ \hline
\multicolumn{2}{|p{20cm}|}{A metodologia proposta não mostra evidências, no artigo, de que fornece suporte para recursos compartilhados e / ou preempções.} \\ \hline
\end{tabular}
}
\end{table}


%**********************************************************
% PUBLICACAO - ID_EXCEL: 083
%**********************************************************
\newpage
\begin{table}[htp] % h:here; t:top; b:bottom; p:page; default:ht
\centering
\caption{Dados extraído da publicação de \cite{Ishihara_2009_a}.}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{|p{3.8cm}|p{16cm}|}
\hline
\multicolumn{1}{|r|}{\textbf{ID}} & Ishihara\_2009\_a \\ \hline
\multicolumn{1}{|r|}{\textbf{Título}} & Real-time power management for a multi-performance processor \\ \hline
\multicolumn{1}{|r|}{\textbf{Autores}} & Ishihara T. \\ \hline
\multicolumn{1}{|r|}{\textbf{Palavras-chave}} & Embedded systems; Low-power design; Microprocessor; Real-time systems \\ \hline
\multicolumn{1}{|r|}{\textbf{Fonte da publicação}} & 2009 International SoC Design Conference, ISOCC 2009 \\ \hline
\multicolumn{1}{|r|}{\textbf{Editora}} & IEEE \\ \hline
\multicolumn{1}{|r|}{\textbf{Ano da publicação}} & 2009 \\ \hline \hline

\multicolumn{2}{|c|}{\textbf{Resumo da publicação}} \\ \hline
\multicolumn{2}{|p{20cm}|}{O autor propõe uma metodologia baseada em uma nova arquitetura contendo vários núcleos de processamento, chamada \textit{Architecture of Multi-Performance Processor}, onde cada núcleo trabalha em uma frequência e tensão específica. Dessa forma, o processador não perde tempo chaveando tensões e frequência, que são em média na casa das centenas de microsegundos. Essa arquitetura quando integrada a técnica DVFS intra-tarefa permite maximizar os ganhos de economiza de energia, através da diminuição dos  \textit{overheads} da técnica DVFS, permitindo fazer chaveamentos de tensão e frequência na casa dos 1.5 microsegundos e dissipando apenas 10 nano-joules. Essa metodologia, reduziu cerca de 25\% de energia em comparação com a técnica DVS convencional do processador.} \\ \hline \hline

\multicolumn{1}{|r|}{\textbf{Método(s) utilizados}} & DVFS Intra-Task; \\ \hline
\multicolumn{1}{|r|}{\textbf{Ferramenta(s)}} & {O autor utilizou a ferramenta RTL Simulation. \newline

O autor utilizou os Benchmarks: \newline
- Adpcm decoder (\textit{Adaptive Differential Pulse Code Modulation}) \newline
- JPEG encoder \newline
- MPEG2 encoder } \\ \hline \hline

\multicolumn{2}{|c|}{\textbf{Impacto (positivo x negativo)}} \\ \hline
\multicolumn{2}{|p{20cm}|}{O artigo apresentou como ponto positivo uma nova proposta de arquitetura para o processador que integrada a técnica DVFS intra-tarefa maximiza os ganhos de economia de energia através da diminuição dos \textit{overheads}. Como pontos negativos, talvez seja uma arquitetura mais cara, pois necessite de mais componentes como memória secundária, caches para cada núcleo de processamento e de um software mais específico e robusto para realizar todo esse gerenciamento.} \\ \hline \hline

\multicolumn{2}{|c|}{\textbf{Validação do método}} \\ \hline
\multicolumn{2}{|p{20cm}|}{A validação da metodologia ocorreu pelo uso de ferramentas de simulação e benchmarks presentes na literatura.} \\ \hline \hline

\multicolumn{2}{|c|}{\textbf{Limitações do método}} \\ \hline
\multicolumn{2}{|p{20cm}|}{Não mostrou nenhum resultado envolvendo várias tarefas e nem levou em consideração preempções.} \\ \hline \hline

\multicolumn{2}{|c|}{\textbf{Integração de métodos}} \\ \hline
\multicolumn{2}{|p{20cm}|}{Não se aplica} \\ \hline \hline

\multicolumn{2}{|c|}{\textbf{Modo de aplicação do método}} \\ \hline
\multicolumn{2}{|p{20cm}|}{Offline} \\ \hline \hline

\multicolumn{2}{|c|}{\textbf{Perspectivas futuras}} \\ \hline
\multicolumn{2}{|p{20cm}|}{Como perspectivas futuras, o autor visa melhorar o sistema de cache da sua arquitetura, pois hoje não está prevendo cache de dados, somente cache de instruções.} \\ \hline \hline

\multicolumn{2}{|c|}{\textbf{Comentários}} \\ \hline
\multicolumn{2}{|p{20cm}|}{A metodologia proposta não mostra evidências, no artigo, de que fornece suporte para recursos compartilhados e / ou preempções.} \\ \hline
\end{tabular}
}
\end{table}


%**********************************************************
% PUBLICACAO - ID_EXCEL: 068
%**********************************************************
\newpage
\begin{table}[htp] % h:here; t:top; b:bottom; p:page; default:ht
\centering
\caption{Dados extraído da publicação de \cite{Mohan_2010_a}.}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{|p{3.8cm}|p{16cm}|}
\hline
\multicolumn{1}{|r|}{\textbf{ID}} & Mohan\_2010\_a \\ \hline
\multicolumn{1}{|r|}{\textbf{Título}} & Parametric timing analysis and its application to dynamic voltage scaling \\ \hline
\multicolumn{1}{|r|}{\textbf{Autores}} & Mohan S., Mueller F., Root M., Hawkins W., Healy C., Whalley D., Vivancos E. \\ \hline
\multicolumn{1}{|r|}{\textbf{Palavras-chave}} & Dynamic voltage scaling; Real-time systems; Timing analysis; Worst-case execution time \\ \hline
\multicolumn{1}{|r|}{\textbf{Fonte da publicação}} & Transactions on Embedded Computing Systems \\ \hline
\multicolumn{1}{|r|}{\textbf{Editora}} & ACM \\ \hline
\multicolumn{1}{|r|}{\textbf{Ano da publicação}} & 2010 \\ \hline \hline

\multicolumn{2}{|c|}{\textbf{Resumo da publicação}} \\ \hline
\multicolumn{2}{|p{20cm}|}{Os autores propõem um metodologia que remove as restrições sobre as invariantes de \textit{loops} através de analises paramétricas, com o objetivo de maximizar a identificação dos tempos de folga das tarefas e minimizar o consumo de energia do processador. Dessa forma, os ganhos dessa abordagem está diretamente relacionado com a redução do número de interações dos \textit{loops} mapeados dentro das aplicações.} \\ \hline \hline

\multicolumn{1}{|r|}{\textbf{Método(s) utilizados}} & DVFS Intra-Task; DVFS Inter-Task; Control Flow Graph (CFG); Loop-Invariant; \\ \hline
\multicolumn{1}{|r|}{\textbf{Ferramenta(s)}} & {Os autores utilizaram as ferramentas: \newline
- SimpleScalar processor simulator (Utilizada pelos autores) \newline
- Preprocesses gcc-generated PISA assembly (Utilizada pelos autores) \newline
- FAST framework (Citada pelos autores) \newline
- VISA framework (Citada pelos autores) \newline

C Benchmarks: \newline
- adpcm (\textit{Adaptive Differential Pulse Code Modulation}) \newline
- cnt (\textit{Sum and count of positive and negative numbers in an array}) \newline
- lms (\textit{An LMS adaptive signal enhancement}) \newline
- mm (\textit{Matrix Multiplication}) } \\ \hline \hline

\multicolumn{2}{|c|}{\textbf{Impacto (positivo x negativo)}} \\ \hline
\multicolumn{2}{|p{20cm}|}{O artigo apresentou como ponto positivo uma metodologia que mostra como aplicar técnicas de invariante de \textit{loop} no contexto de sistemas de tempo real para diminuir o consumo de energia e os tempos de folga das tarefas. Como ponto negativo, os autores relatam que precisa melhorar sua metodologia para lidar com casos especiais que tenha um número menor de iterações dentro dos \textit{loops}.} \\ \hline \hline

\multicolumn{2}{|c|}{\textbf{Validação do método}} \\ \hline
\multicolumn{2}{|p{20cm}|}{A validação da metodologia ocorreu pelo uso de ferramentas de simulação e benchmarks presentes na literatura. Além disso, comparou os resultados experimentais obtidos com outras abordagens presentes na literatura.} \\ \hline \hline

\multicolumn{2}{|c|}{\textbf{Limitações do método}} \\ \hline
\multicolumn{2}{|p{20cm}|}{Não mostrou nenhum resultado experimental envolvendo várias tarefas e não deixou claro como a metodologia lidar com as preempções.} \\ \hline \hline

\multicolumn{2}{|c|}{\textbf{Integração de métodos}} \\ \hline
\multicolumn{2}{|p{20cm}|}{Foram integradas as técnicas: \textit{inter-task}, \textit{intra-task} e \textit{loop-invariant}} \\ \hline \hline

\multicolumn{2}{|c|}{\textbf{Modo de aplicação do método}} \\ \hline
\multicolumn{2}{|p{20cm}|}{Híbrida} \\ \hline \hline

\multicolumn{2}{|c|}{\textbf{Perspectivas futuras}} \\ \hline
\multicolumn{2}{|p{20cm}|}{Como perspectivas futuras, os autores visam melhorar seu método para lidar com um número menor de iterações dentro dos \textit{loops}.} \\ \hline \hline

\multicolumn{2}{|c|}{\textbf{Comentários}} \\ \hline
\multicolumn{2}{|p{20cm}|}{A metodologia mostra indícios de que dá suporte a preempções entre tarefas, mas não deixa claro como é feito. Quanto a recursos compartilhados, a metodologia não dá suporte.} \\ \hline
\end{tabular}
}
\end{table}


%**********************************************************
% PUBLICACAO - ID_EXCEL: 056
%**********************************************************
\newpage
\begin{table}[htp] % h:here; t:top; b:bottom; p:page; default:ht
\centering
\caption{Dados extraído da publicação de \cite{Tatematsu_2011_a}.}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{|p{3.8cm}|p{16cm}|}
\hline
\multicolumn{1}{|r|}{\textbf{ID}} & Tatematsu\_2011\_a \\ \hline
\multicolumn{1}{|r|}{\textbf{Título}} & Checkpoint extraction using execution traces for intra-task DVFS in embedded systems \\ \hline
\multicolumn{1}{|r|}{\textbf{Autores}} & Tatematsu T., Takase H., Zeng G., Tomiyama H., Takada H. \\ \hline
\multicolumn{1}{|r|}{\textbf{Palavras-chave}} & DVFS; Embedded system; Execution trace; Low energy \\ \hline
\multicolumn{1}{|r|}{\textbf{Fonte da publicação}} & Proceedings - 2011 6th IEEE International Symposium on Electronic Design, Test and Application, DELTA 2011 \\ \hline
\multicolumn{1}{|r|}{\textbf{Editora}} & IEEE \\ \hline
\multicolumn{1}{|r|}{\textbf{Ano da publicação}} & 2011 \\ \hline \hline

\multicolumn{2}{|c|}{\textbf{Resumo da publicação}} \\ \hline
\multicolumn{2}{|p{20cm}|}{Os autores propõem uma metodologia que analisa o código fonte da aplicação e lista todos os possíveis locais para a inserção de pontos de controle (também chamado pelos autores de \textit{checkpoints}). Em seguida, todos esses pontos são analisado e os que não trazem ganhos energéticos são removidos. Por fim, a metodologia compara essa listagem de pontos de controle com uma tabela RWCEC (em inglês, \textit{Remaining Worst Case Execution Cycles}), também extraída da aplicação, para então calcular as tensões e frequências que deverão ser utilizadas no processador.} \\ \hline \hline

\multicolumn{1}{|r|}{\textbf{Método(s) utilizados}} & DVFS Intra-Task; Control Flow Graph (CFG); \\ \hline
\multicolumn{1}{|r|}{\textbf{Ferramenta(s)}} & {Os autores utilizaram a ferramenta SimpleScalarARM (Disponível em: \href{http://www.simplescalar.com/}{http://www.simplescalar.com/}) e o benchmark MediaBench (Disponível em: \href{http://dl.acm.org/citation.cfm?id=266800.266832}{http://dl.acm.org/citation.cfm?id=266800.266832}).} \\ \hline \hline

\multicolumn{2}{|c|}{\textbf{Impacto (positivo x negativo)}} \\ \hline
\multicolumn{2}{|p{20cm}|}{O artigo apresentou como ponto positivo uma metodologia faz uma análise do código fonte da tarefa com base no RWCEC para saber os pontos ideais no código onde devem ser inseridos os pontos de controle (ou \textit{checkpoints}), contribuindo significativamente para a melhoraria da aplicação da técnica DVFS intra-tarefa. Como ponto negativo, a metodologia precisar ser melhorada, pois os resultados dos seus experimentos mostraram que a inserção de alguns \textit{checkpoint} na aplicação podem causar a perda de alguns deadlines.} \\ \hline \hline

\multicolumn{2}{|c|}{\textbf{Validação do método}} \\ \hline
\multicolumn{2}{|p{20cm}|}{A validação da metodologia ocorreu pelo uso de benchmarks presentes na literatura, onde compara os resultados obtidos com a abordagem DVFS inter-tarefa.} \\ \hline \hline

\multicolumn{2}{|c|}{\textbf{Limitações do método}} \\ \hline
\multicolumn{2}{|p{20cm}|}{Necessário fazer um estudos mais detalhado sobre os checkpoints, pois alguns experimentos resultaram na violação das restrições temporais das tarefas. Não mostrou nenhum resultado envolvendo várias tarefas e nem preempções.} \\ \hline \hline

\multicolumn{2}{|c|}{\textbf{Integração de métodos}} \\ \hline
\multicolumn{2}{|p{20cm}|}{Não se aplica} \\ \hline \hline

\multicolumn{2}{|c|}{\textbf{Modo de aplicação do método}} \\ \hline
\multicolumn{2}{|p{20cm}|}{\textit{Offline}} \\ \hline \hline

\multicolumn{2}{|c|}{\textbf{Perspectivas futuras}} \\ \hline
\multicolumn{2}{|p{20cm}|}{Como perspectivas futuras, os autores visam integrar métodos para lidar com as perdas de deadlines e melhorar a eficiência do algoritmo de extração de \textit{checkpoints}.} \\ \hline \hline

\multicolumn{2}{|c|}{\textbf{Comentários}} \\ \hline
\multicolumn{2}{|p{20cm}|}{A metodologia proposta não mostra evidências, no artigo, de que fornece suporte para recursos compartilhados e / ou preempções.} \\ \hline
\end{tabular}
}
\end{table}


%**********************************************************
% PUBLICACAO - ID_EXCEL: 053
%**********************************************************
\newpage
\begin{table}[htp] % h:here; t:top; b:bottom; p:page; default:ht
\centering
\caption{Dados extraído da publicação de \cite{Takase_2011_a}.}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{|p{3.8cm}|p{16cm}|}
\hline
\multicolumn{1}{|r|}{\textbf{ID}} & Takase\_2011\_a \\ \hline
\multicolumn{1}{|r|}{\textbf{Título}} & An integrated optimization framework for reducing the energy consumption of embedded real-time applications \\ \hline
\multicolumn{1}{|r|}{\textbf{Autores}} & Takase H., Zeng G., Gauthier L., Kawashima H., Atsumi N., Tatematsu T., Kobayashi Y., Kohara S., Koshiro T., Ishihara T., Tomiyama H., Takada H. \\ \hline
\multicolumn{1}{|r|}{\textbf{Palavras-chave}} & development environment; embedded application; energy optimization \\ \hline
\multicolumn{1}{|r|}{\textbf{Fonte da publicação}} & Proceedings of the International Symposium on Low Power Electronics and Design					 \\ \hline
\multicolumn{1}{|r|}{\textbf{Editora}} & IEEE \\ \hline
\multicolumn{1}{|r|}{\textbf{Ano da publicação}} & 2011 \\ \hline \hline

\multicolumn{2}{|c|}{\textbf{Resumo da publicação}} \\ \hline
\multicolumn{2}{|p{20cm}|}{Os autores desenvolvem um \textit{framework} com o objetivo de melhor realizar o chaveamento entre performance e consumo de energia do processador. As configurações ótimas do processador são definidas de acordo com cada etapa de execução da tarefa. Além disso, esse \textit{framework} aplica técnicas de otimização sobre a alocação de memória da aplicação, visando diminuir \textit{overheads} de IO (em inglês, \textit{Input and Output}). Dessa forma, todas as características e comportamento da aplicação são analisados tando do ponto de vista inter quanto intra tarefa. Os resultados dessa análise, resultam na otimização de energia em tempo de execução de acordo com o comportamento da aplicação. Os resultados experimentais utilizando um sistema de vídeo conferencia conseguiram reduzir em média o consumo de energia em 44.9\% em comparação com outros estudos de caso criados pelo próprio autor.} \\ \hline \hline

\multicolumn{1}{|r|}{\textbf{Método(s) utilizados}} & DVFS Intra-Task; DVFS Inter-Task; Control Flow Graph (CFG); \\ \hline
\multicolumn{1}{|r|}{\textbf{Ferramenta(s)}} & {Os autores implementaram um framework, mas não deixa claro o nome da ferramenta criada (talvez seja toolchain). \newline

Lista dos Benchmarks utilizados: \newline
- Xvid MPEG-4 video codec \newline
- FFmpeg library } \\ \hline \hline

\multicolumn{2}{|c|}{\textbf{Impacto (positivo x negativo)}} \\ \hline
\multicolumn{2}{|p{20cm}|}{O artigo apresentou como ponto positivo uma metodologia que integra otimização inter-tarefa e intra-tarefa, modificando o código fonte das tarefas de tempo real, principalmente através de \textit{checkpoints} (pontos de controle). Além de propor otimizações na alocação de memória. Como pontos negativos, os autores não mostraram nenhum estudo sobre os overheads inseridos pelo framework.} \\ \hline \hline

\multicolumn{2}{|c|}{\textbf{Validação do método}} \\ \hline
\multicolumn{2}{|p{20cm}|}{A validação da abordagem ocorreu por meio do uso de casos de testes criados pelos próprios autores.} \\ \hline \hline

\multicolumn{2}{|c|}{\textbf{Limitações do método}} \\ \hline
\multicolumn{2}{|p{20cm}|}{A metodologia não mostra estudos detalhados sobre os \textit{overheads} gerados dentro das tarefas.} \\ \hline \hline

\multicolumn{2}{|c|}{\textbf{Integração de métodos}} \\ \hline
\multicolumn{2}{|p{20cm}|}{Não se aplica} \\ \hline \hline

\multicolumn{2}{|c|}{\textbf{Modo de aplicação do método}} \\ \hline
\multicolumn{2}{|p{20cm}|}{Híbrida} \\ \hline \hline

\multicolumn{2}{|c|}{\textbf{Perspectivas futuras}} \\ \hline
\multicolumn{2}{|p{20cm}|}{Extender o framework para ambientes com mais de um processador.} \\ \hline \hline

\multicolumn{2}{|c|}{\textbf{Comentários}} \\ \hline
\multicolumn{2}{|p{20cm}|}{O artigo mostra indícios de que dá suporte a preempções, mas não deixa claro no artigo como é feito, e não dá suporte a recursos compartilhados.} \\ \hline
\end{tabular}
}
\end{table}


%**********************************************************
% PUBLICACAO - ID_EXCEL: 052
%**********************************************************
\newpage
\begin{table}[htp] % h:here; t:top; b:bottom; p:page; default:ht
\centering
\caption{Dados extraído da publicação de \cite{Yuan_2011_a}.}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{|p{3.8cm}|p{16cm}|}
\hline
\multicolumn{1}{|r|}{\textbf{ID}} & Yuan\_2011\_a \\ \hline
\multicolumn{1}{|r|}{\textbf{Título}} & TALk: A temperature-aware leakage minimization technique for real-time systems \\ \hline
\multicolumn{1}{|r|}{\textbf{Autores}} & Yuan L., Leventhal S.R., Gu J., Qu G. \\ \hline
\multicolumn{1}{|r|}{\textbf{Palavras-chave}} & Dynamic voltage scaling; low power; real-time systems; temperature-aware design \\ \hline
\multicolumn{1}{|r|}{\textbf{Fonte da publicação}} & IEEE Transactions on Computer-Aided Design of Integrated Circuits and Systems \\ \hline
\multicolumn{1}{|r|}{\textbf{Editora}} & IEEE \\ \hline
\multicolumn{1}{|r|}{\textbf{Ano da publicação}} & 2011 \\ \hline \hline

\multicolumn{2}{|c|}{\textbf{Resumo da publicação}} \\ \hline
\multicolumn{2}{|p{20cm}|}{Os autores propõem um algoritmo de escalonamento intra-tarefa que visa diminuir a temperatura do processador e minimizar o consumo de energia em sistema de tempo real. Essa técnica foi chamada de \textit{TALk} (em inglês, \textit{Temperature- Aware Leakage}). A ideia básica do algoritmo é aumentar a frequência quando a temperatura do chip estiver baixa ou quando a carga de trabalho for alta e colocar o processador em baixo consumo de energia quando a temperatura do chip estiver alta ou com carga de trabalho leve. Para fazer isso, o algoritmo \textit{TALk} foi dividida em duas partes: (1) A \textit{Offline}, que usa métodos de programação dinâmica para alcançar os melhores níveis de economia de energia e de temperatura; (2) O \textit{Online} tem como objetivo determinar o modo de operação do processador com base na sua temperatura corrente e na quantidade de ciclos remanescentes das tarefas em execução. Com esse algoritmo os autores conseguiram melhorar a economia de energia em cerca de 18\% em comparação com a técnica DVS tradicional.} \\ \hline \hline

\multicolumn{1}{|r|}{\textbf{Método(s) utilizados}} & DVFS Intra-Task; \\ \hline
\multicolumn{1}{|r|}{\textbf{Ferramenta(s)}} & {Os autores não mencionaram nenhuma ferramenta específica, mas utilizaram 4 Benchmark para geração dos 11 casos de teste utilizados para realização dos experimentos. \newline

Lista dos Benchmarks utilizados pelos autores:\newline
- MPEG4 \textit{media encoding} (Disponível em: \href{http://ieeexplore.ieee.org/xpl/articleDetails.jsp? arnumber=914596}{http://ieeexplore.ieee.org/xpl/articleDetails.jsp? arnumber=914596})\newline
- \textit{Hartstone suite} (Disponível em: \href{http://ieeexplore.ieee.org/xpl/articleDetails.jsp? arnumber=766516}{http://ieeexplore.ieee.org/xpl/articleDetails.jsp? arnumber=766516})\newline
- \textit{ADSL standard's initialization sequences} (Disponível em: \href{http://ieeexplore.ieee.org/xpl/ articleDetails.jsp?arnumber=953271}{http://ieeexplore.ieee.org/xpl/ articleDetails.jsp?arnumber=953271})\newline
- Os outros foram gerados artificialmente pelos autores.} \\ \hline \hline

\multicolumn{2}{|c|}{\textbf{Impacto (positivo x negativo)}} \\ \hline
\multicolumn{2}{|p{20cm}|}{O artigo apresentou como ponto positivo uma metodologia onde é possível diminuir o consumo de energia do processador e ao mesmo tempo controlar a sua temperatura. Como ponto negativo, os autores falam que para alguns benchmarks o algoritmo off-line pode violar as restrições temporais de algumas tarefas.} \\ \hline \hline

\multicolumn{2}{|c|}{\textbf{Validação do método}} \\ \hline
\multicolumn{2}{|p{20cm}|}{\textcolor{red}{ERRADO: A validação da abordagem ocorreu por meio do uso de Benchmarks utilizado por outros trabalhos presentes na literatura. Além de comparar os resultados obtidos experimentalmente com outros trabalhos presentes na literatura.}} \\ \hline \hline

\multicolumn{2}{|c|}{\textbf{Limitações do método}} \\ \hline
\multicolumn{2}{|p{20cm}|}{Os autores mencionam que o algoritmo \textit{offline} pode violar as restrições temporais de algumas tarefas.} \\ \hline \hline

\multicolumn{2}{|c|}{\textbf{Integração de métodos}} \\ \hline
\multicolumn{2}{|p{20cm}|}{Não se aplica} \\ \hline \hline

\multicolumn{2}{|c|}{\textbf{Modo de aplicação do método}} \\ \hline
\multicolumn{2}{|p{20cm}|}{Híbrida} \\ \hline \hline

\multicolumn{2}{|c|}{\textbf{Perspectivas futuras}} \\ \hline
\multicolumn{2}{|p{20cm}|}{Melhorar o algoritmo offline para resolver o problema de violação de restrições temporais de algumas tarefas.} \\ \hline \hline

\multicolumn{2}{|c|}{\textbf{Comentários}} \\ \hline
\multicolumn{2}{|p{20cm}|}{A metodologia proposta não mostra evidências, no artigo, de que fornece suporte para recursos compartilhados e / ou preempções.} \\ \hline
\end{tabular}
}
\end{table}


%**********************************************************
% PUBLICACAO - ID_EXCEL: 033
%**********************************************************
\newpage
\begin{table}[htp] % h:here; t:top; b:bottom; p:page; default:ht
\centering
\caption{Dados extraído da publicação de \cite{Cohen_2012_a}.}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{|p{3.8cm}|p{16cm}|}
\hline
\multicolumn{1}{|r|}{\textbf{ID}} & Cohen\_2012\_a \\ \hline
\multicolumn{1}{|r|}{\textbf{Título}} & A Car Racing Based Strategy for the Dynamic Voltage and Frequency Scaling Technique \\ \hline
\multicolumn{1}{|r|}{\textbf{Autores}} & David Cohen, Eduardo Valentin, Raimundo Barreto, Horácio Oliveira, and Lucas Cordeiro \\ \hline
\multicolumn{1}{|r|}{\textbf{Palavras-chave}} & Dynamic voltage and frequency scaling; Energy consumption optimization; Low energy consumption; Real-time application; Real-time tasks; Worst-case execution; Buffer storage; Energy utilization; Industrial electronics \\ \hline
\multicolumn{1}{|r|}{\textbf{Fonte da publicação}} & IEEE International Symposium on Industrial Electronics \\ \hline
\multicolumn{1}{|r|}{\textbf{Editora}} & IEEE \\ \hline
\multicolumn{1}{|r|}{\textbf{Ano da publicação}} & 2012 \\ \hline \hline

\multicolumn{2}{|c|}{\textbf{Resumo da publicação}} \\ \hline
\multicolumn{2}{|p{20cm}|}{Os autores apresentam uma nova política de escalonamento de tarefas de tempo real, que leva em consideração preempções. Esse nova metodologia consegue economizar energia mesmo executando as tarefas no seu pior caso. Em resumo, o autor faz uma analogia entre escalonador e suas tarefas, com uma corrida de carros, onde o objetivo da corrida é que todos os carros (uma analogia as tarefas) cheguem juntos no final, utilizando as menores velocidades (uma analogia a tensões e frequências do processador) sem que nenhuma premissa temporal seja violada. Essa nova política de escalonamento foi experimentada apenas em ambiente simulado e utilizando casos de teste gerados pelos próprios autores.} \\ \hline \hline

\multicolumn{1}{|r|}{\textbf{Método(s) utilizados}} & DVFS Intra-Task; Control flow graph (CFG); \\ \hline
\multicolumn{1}{|r|}{\textbf{Ferramenta(s)}} & {O autor não utilizou nenhuma ferramenta, mas nas referências é citada a ferramenta COPPER Framework.} \\ \hline \hline

\multicolumn{2}{|c|}{\textbf{Impacto (positivo x negativo)}} \\ \hline
\multicolumn{2}{|p{20cm}|}{\textcolor{red}{MELHORAR E SIMPLIFICAR TEXTO: O artigo apresentou impactos positivos uma nova metodologia de escalonamento de tarefas para sistemas de tempo real levando em consideração as preempções, o respeito as restrições temporais e o baixo consumo de energia, mesmo executando o pior caso de execução das tarefas.} Como impacto negativo, a metodologia foi valida apenas com simulações, não foi utilizado nenhum benchmark ou casos de testes reais para validação do método proposto.} \\ \hline \hline

\multicolumn{2}{|c|}{\textbf{Validação do método}} \\ \hline
\multicolumn{2}{|p{20cm}|}{A validação da abordagem ocorreu por meio de exemplos propostos pelos próprios autores, onde estes exemplos exploraram várias tarefas em execução, preempções e o baixo consumo de energia do processador.} \\ \hline \hline

\multicolumn{2}{|c|}{\textbf{Limitações do método}} \\ \hline
\multicolumn{2}{|p{20cm}|}{\textcolor{red}{ERRADO: O método proposto foi aplicado apenas em ambiente simulado. Talvez seja necessário fazer um estudo mais detalhado para saber o real impacto dos overheads gerados por essa metodologia.}} \\ \hline \hline

\multicolumn{2}{|c|}{\textbf{Integração de métodos}} \\ \hline
\multicolumn{2}{|p{20cm}|}{Não se aplica} \\ \hline \hline

\multicolumn{2}{|c|}{\textbf{Modo de aplicação do método}} \\ \hline
\multicolumn{2}{|p{20cm}|}{Online} \\ \hline \hline

\multicolumn{2}{|c|}{\textbf{Perspectivas futuras}} \\ \hline
\multicolumn{2}{|p{20cm}|}{Pretendem realizar experimentos com estudos de casos reais da industria e implementar o método proposto em uma plataforma real, através da inclusão de uma nova camada entre a aplicação e o sistema operacional.} \\ \hline \hline

\multicolumn{2}{|c|}{\textbf{Comentários}} \\ \hline
\multicolumn{2}{|p{20cm}|}{A metodologia deixa clara que dá suporte a preempções. Quanto aos recursos compartilhados, eles são previstos apenas no teste de escalonabilidade do modelo de tarefas proposto e não mostra nos resultados experimentos modelos de tarefas que compartilhem recursos.} \\ \hline
\end{tabular}
}
\end{table}


%**********************************************************
% PUBLICACAO - ID_EXCEL: 027
%**********************************************************
\newpage
\begin{table}[htp] % h:here; t:top; b:bottom; p:page; default:ht
\centering
\caption{Dados extraído da publicação de \cite{Seo_Seo_Kim_2012_a}.}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{|p{3.8cm}|p{16cm}|}
\hline
\multicolumn{1}{|r|}{\textbf{ID}} & Seo\_Seo\_Kim\_2012\_a \\ \hline
\multicolumn{1}{|r|}{\textbf{Título}} & Algorithms for combined inter- and intra-task dynamic voltage scaling \\ \hline
\multicolumn{1}{|r|}{\textbf{Autores}} & Seo H., Seo J., Kim T. \\ \hline
\multicolumn{1}{|r|}{\textbf{Palavras-chave}} & dynamic voltage scaling (DVS); embedded systems; power saving \\ \hline
\multicolumn{1}{|r|}{\textbf{Fonte da publicação}} & Computer Journal \\ \hline
\multicolumn{1}{|r|}{\textbf{Editora}} & Oxford University Press on behalf of The British Computer Society \\ \hline
\multicolumn{1}{|r|}{\textbf{Ano da publicação}} & 2012 \\ \hline \hline

\multicolumn{2}{|c|}{\textbf{Resumo da publicação}} \\ \hline
\multicolumn{2}{|p{20cm}|}{Os autores apresentam uma técnica de baixo consumo de energia que se baseia na combinação simultânea entre inter-tarefa e intra-tarefa, também chamada DVS combinado (em inglês, \textit{Combined} DVS - CDVS). Essa nova abordagem leva em consideração o estado do sistema dormindo (em inglês, \textit{Sleep State} - CDVS-S) e não dormindo (em inglês, \textit{No Sleep State} - CDVS-NS). Ela consiste basicamente de 4 etapas: (1) Aplicar a técnica CDVS-NS para determinar os intervalos de execução das tarefas de modo que o consumo total de energia seja minimizado, sem estados de dormindo (\textit{sleep state}); (2) Realizar a análise estática dos blocos de código da tarefa, a fim de identificar os tempos ociosos e as tensões e frequências que deverão ser utilizadas; (3) Combinar os intervalos de tempo salvos na segunda etapa com o maior tempo possível no qual o sistema possa estar no estado ocioso (\textit{idle state}) de forma eficiente; e por último (4) Monitorar dinamicamente todas as instâncias das tarefas em execução que concluíram sua execução antes do prazo final e, em seguida, irá decidir se coloca a tarefa em estado ociosa (\textit{idle state}) ou em estado de dormindo (\textit{sleep state}), dependendo do que for mais econômico energeticamente. Em geral, essa metodologia conseguiu reduzir o consumo de energia em média de 7\% com a técnica CDVS-S e de 12\% com a técnica CDVS-NS em comparação com outros trabalhos presentes na literatura.} \\ \hline \hline

\multicolumn{1}{|r|}{\textbf{Método(s) utilizados}} & DVFS \textit{Intra-Task}; DVFS \textit{Inter-Task}; \\ \hline
\multicolumn{1}{|r|}{\textbf{Ferramenta(s)}} & {O autor utilizou as ferramentas TGFF v 3.0 (usando C++ e suas bibliotecas padrões) e MiBench \textit{benchmarks}.} \\ \hline \hline

\multicolumn{2}{|c|}{\textbf{Impacto (positivo x negativo)}} \\ \hline
\multicolumn{2}{|p{20cm}|}{\textcolor{red}{ERRADO: O artigo apresentou como impacto positivo uma metodologia de baixo consumo de energia que integra as técnicas inter e intra tarefa, que ainda não havia sido relatada na literatura.} Como ponto negativo, os autores não apresentaram nenhum estudo sobre os impactos da integração dessas duas técnicas.} \\ \hline \hline

\multicolumn{2}{|c|}{\textbf{Validação do método}} \\ \hline
\multicolumn{2}{|p{20cm}|}{A validação da abordagem ocorreu por meio de benchmarks, provas matemáticas e comparações dos resultados com outros trabalhos presentes na literatura.} \\ \hline \hline

\multicolumn{2}{|c|}{\textbf{Limitações do método}} \\ \hline
\multicolumn{2}{|p{20cm}|}{É necessário fazer um estudo mais detalhado sobre os reais impactos da integração das técnicas inter e intra tarefa, pois o artigo não deixo claro.} \\ \hline \hline

\multicolumn{2}{|c|}{\textbf{Integração de métodos}} \\ \hline
\multicolumn{2}{|p{20cm}|}{Foi integrado as técnicas inter e intra tarefas (DVFS).} \\ \hline \hline

\multicolumn{2}{|c|}{\textbf{Modo de aplicação do método}} \\ \hline
\multicolumn{2}{|p{20cm}|}{Híbrido.} \\ \hline \hline

\multicolumn{2}{|c|}{\textbf{Perspectivas futuras}} \\ \hline
\multicolumn{2}{|p{20cm}|}{Criar um modelo de economia de energia que leve em consideração outros componentes do sistema com as memórias, interfaces e comportamento das tarefas.} \\ \hline \hline

\multicolumn{2}{|c|}{\textbf{Comentários}} \\ \hline
\multicolumn{2}{|p{20cm}|}{A metodologia proposta não mostra evidências, no artigo, de que fornece suporte para recursos compartilhados e / ou preempções.} \\ \hline
\end{tabular}
}
\end{table}


%**********************************************************
% PUBLICACAO - ID_EXCEL: 019
%**********************************************************
\newpage
\begin{table}[htp] % h:here; t:top; b:bottom; p:page; default:ht
\centering
\caption{Dados extraído da publicação de \cite{Awan_Petters_2012_a}.}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{|p{3.8cm}|p{16cm}|}
\hline
\multicolumn{1}{|r|}{\textbf{ID}} & Awan\_Petters\_2012\_a \\ \hline
\multicolumn{1}{|r|}{\textbf{Título}} & Online Intra-Task Device Scheduling for Hard Real-Time Systems \\ \hline
\multicolumn{1}{|r|}{\textbf{Autores}} & Muhammad Ali Awan, Stefan M. Petters \\ \hline
\multicolumn{1}{|r|}{\textbf{Palavras-chave}} & Battery life; Device scheduling; Energy gain; Hard real-time systems; I/O Device; Large parts; Power saving mechanism; Schedulability; Technology enhancements; Embedded systems; Energy resources; Energy utilization; Interactive computer systems; Scheduling algorithms; Real time systems \\ \hline
\multicolumn{1}{|r|}{\textbf{Fonte da publicação}} & 7th IEEE International Symposium on Industrial Embedded Systems, SIES 2012 - Conference Proceedings \\ \hline
\multicolumn{1}{|r|}{\textbf{Editora}} & IEEE \\ \hline
\multicolumn{1}{|r|}{\textbf{Ano da publicação}} & 2012 \\ \hline \hline

\multicolumn{2}{|c|}{\textbf{Resumo da publicação}} \\ \hline
\multicolumn{2}{|p{20cm}|}{Os autores propõem um algoritmo (online) de escalonamento intra-tarefa, cuja principal funcionalidade é ligar e desligar dispositivos do hardware, permitindo que eles sejam utilizados somente quando necessário. Essa metodologia se aplica a sistemas de tempo real crítico e funciona basicamente explorando os tempos de folga entre as execuções das tarefas, a fim de realizar o melhor gerenciamento dos acionamentos e desligamento dos dispositivos,  melhorando assim a performance de economia de energia do sistema. Os experimentos mostram um ganho de economia de energia acima dos 90\% em comparação com outras técnicas presentes na literatura.} \\ \hline \hline

\multicolumn{1}{|r|}{\textbf{Método(s) utilizados}} & DVFS \textit{Intra-Task}; \\ \hline
\multicolumn{1}{|r|}{\textbf{Ferramenta(s)}} & {Utilizou o simulador SPARTS V 2.0 (\textit{Simulator for Power Aware and Real-Time System}).} \\ \hline \hline

\multicolumn{2}{|c|}{\textbf{Impacto (positivo x negativo)}} \\ \hline
\multicolumn{2}{|p{20cm}|}{O artigo apresentou como impacto positivo uma metodologia para gerenciar os dispositivos do sistema sobre demanda, permitindo assim acioná-los somente quando necessário. No entanto, o impacto negativo dessa abordagem está nos \textit{overheads} adicionados nas premissas temporais de cada tarefa.} \\ \hline \hline

\multicolumn{2}{|c|}{\textbf{Validação do método}} \\ \hline
\multicolumn{2}{|p{20cm}|}{A validação da abordagem ocorreu por meio de exemplos propostos no próprio artigo, onde estes exemplos exploraram várias tarefas em execução, levando em consideração WCETs, deadlines, intervalo mínimo de chegada entre tarefas e os dispositivos utilizados por cada uma delas.} \\ \hline \hline

\multicolumn{2}{|c|}{\textbf{Limitações do método}} \\ \hline
\multicolumn{2}{|p{20cm}|}{O método proposto foi aplicado apenas em ambiente simulado, prever apenas o uso de um dispositivo e não leva em consideração o compartilhamento de dispositivos entre tarefas.} \\ \hline \hline

\multicolumn{2}{|c|}{\textbf{Integração de métodos}} \\ \hline
\multicolumn{2}{|p{20cm}|}{Não se aplica} \\ \hline \hline

\multicolumn{2}{|c|}{\textbf{Modo de aplicação do método}} \\ \hline
\multicolumn{2}{|p{20cm}|}{Online} \\ \hline \hline

\multicolumn{2}{|c|}{\textbf{Perspectivas futuras}} \\ \hline
\multicolumn{2}{|p{20cm}|}{Pretendem melhorar a aplicabilidade deste método para sistemas mais versáteis, permitindo que seja possível compartilhar dispositivos entre tarefas e aumentar o uso de dispositivos por tarefa.} \\ \hline \hline

\multicolumn{2}{|c|}{\textbf{Comentários}} \\ \hline
\multicolumn{2}{|p{20cm}|}{A metodologia proposta dá suporte a recursos compartilhados, mas cada recurso é utilizado apenas por uma única tarefa por vez. Em relação ao suporte a preempções, o artigo mostra algumas deduções formais, mas não deixa claro se dá suporte.} \\ \hline
\end{tabular}
}
\end{table}

